Asymptotic String Compactifications; Periods, flux potentials, and the swampland

In this thesis we have studied various applications of asymptotic Hodge theory in string compactifications. This mathematical framework captures how physical couplings of the resulting effective theories behave near field space boundaries where the internal Calabi-Yau manifold degenerates. Below we summarize the three parts in which this thesis is divided. Part I introduces the techniques from asymptotic Hodge theory we used throughout this thesis. We review the results of the nilpotent orbit theorem of Schmid and the multi-variable sl(2)-orbit theorem of Cattani, Kaplan and Schmid. This discussion is tailored to applications in string compactifications, explaining how to describe important physical couplings such as K\"ahler potentials and flux superpotentials near boundaries in moduli spaces. Part II discusses a geometrical application with the construction of general models for asymptotic periods. Taking the constraints imposed by asymptotic Hodge theory as consistency principles, we develop new methods for constructing these periods. We explicitly carry out our program for all possible one- and two-moduli boundaries. Part III discusses two applications of asymptotic Hodge theory in string compactifications. The first investigates bounds put by the Weak Gravity Conjecture in the setting of 4d $\mathcal{N}=2$ supergravity theories arising from Type IIB Calabi-Yau compactifications. The second application studies flux potentials in asymptotic regimes in complex structure moduli space, where we develop two schemes for moduli stabilization. The first scheme sets up an approximation procedure for finding flux vacua divided in three steps: the sl(2)-approximation, the nilpotent orbit approximation, and the fully corrected result. The second scheme constructs flux vacua with a small flux superpotential by using essential exponential corrections controlled by asymptotic Hodge theory.

==> Stabilization.tex <==



%In order to obtain phenomenologically interesting effective theories from string theory, it is vital to ensure that neutral scalar fields have a sufficiently large mass in order to not contradict fifth force bounds.The most prominent way to achieve this is by considering string theory solutions that include background fluxes \cite{Grana:2005jc,Douglas:2006es,Blumenhagen:2006ci}. Such fluxes can, for example, fix the complex-structure of the compactifications geometry and thus give potential complex-structure deformation moduli a mass. The most prominent and best understood scenario where this happens in a controlled way are Type IIB orientifold compactifications with O3/O7-planes and their more general F-theory counterparts. In these settings the precise way how moduli stabilization occurs has been studied for many examples by explicitly constructing the compact Calabi-Yau geometry, specifying a flux, and deriving the scalar potential for the complex-structure moduli. However, it is difficult to draw general conclusions from such specific examples, which makes it hard to interpret the findings in these special cases in a broader context. 

%In recent years the swampland program, which aims at identifying general principles that every effective theory consistent with quantum gravity has to satisfy, has forced us to develop novel approaches to study general properties of effective theories arising from string theory. In particular, the well-defined Type IIB and F-theory settings, are a perfect testing ground for many swampland conjectures. This does require, however, to move beyond studying specific examples and rather uncover the universal structures appearing in all such compactifications. While this is a challenging task in general, it has recently become clear that it becomes tractable if we focus on the asymptotic regimes of the field space and apply the powerful tools of asymptotic Hodge theory. Following \cite{Grimm:2019ixq} we will call the such scenarios  \textit{asymptotic flux compactifications} in the following. To introduce them in more detail, we recall that the relevant compactification geometries for Type IIB and F-theory settings without fluxes are Calabi-Yau three- and fourfolds, respectively. These manifolds admit a deformation space known as the complex-structure moduli space, which parametrizes the allowed choices of complex-structures on these geometries.     It is crucial to realize that this moduli space is not compact, but rather has boundaries and thus associated asymptotic regions. Asymptotic Hodge theory gives a detailed understanding of how the Hodge decomposition of forms behaves in these regions and provides a dictionary for how data associated to an individual boundary component determines the asymptotic form of the flux-induced scalar potential. 

In this work we suggest that the mathematical results of asymptotic Hodge theory provide 
a systematic algorithm to perform moduli stabilization near any boundary of moduli space. Finding 
flux vacua requires to solve a self-duality condition on the fluxes involving the Hodge star. The moduli 
dependence of the Hodge star is, in general, a very complicated transcendental function that depends 
on many details of the compactification geometry. However, in the asymptotic regime there exists an approximation 
scheme to extract the moduli dependence in essentially three steps: (1) the sl(2)-approximation, (2) the nilpotent orbit 
approximation, (3) the fully corrected result. In steps (1) and (2) a certain set of corrections is consistently neglected, turning the extremely hard problem of finding flux vacua into a tractable algebraic problem. It is important to stress that it is a very non-trivial fact that such approximations exist in all asymptotic regimes. In particular, 
this is remarkable because it was shown in \cite{Bastian:2021eom} that in almost all asymptotic regimes exponential corrections are essential 
when deriving the Hodge star from the period integrals of the unique $(3,0)$-form or $(4,0)$-form 
of the Calabi-Yau manifold. The determination of the approximated Hodge star is non-trivial, 
but can be done explicitly for any given example following the algorithms that we discuss 
in detail in this work. 

The most involved computations are needed to determine the sl(2)-approximation. The crucial 
result of \cite{CKS} is that in any boundary regime in which the moduli satisfy a certain
hierarchy a number of $n$ commuting sl$(2,\bbC)$ algebras and a boundary Hodge decomposition 
can be determined. This data in turn determines a split of the flux space and the asymptotic form 
of the Hodge star operator used, for example, in the flux vacuum conditions. We collect some intuitive arguments why such structures emerge 
at the boundary and discuss the step-by-step procedure to construct the sl(2)s and the boundary 
Hodge decomposition. This algorithm has already been given in \cite{Grimm:2018cpv} and can be extracted from the 
original works \cite{CKS, Kato}. The approach is iterative in the number of moduli that admit a hierarchy and 
uses solely linear algebra, even though in a somewhat intricate way. Therefore, it can be easily 
implemented on a computer and any given example can be evaluate very rapidly. We discuss 
one example in detail and present all the asymptotic data needed in the sl(2)-approximation. Remarkably,
the sl(2)-approximation can also be used abstractly, i.e.~one can parametrise unknown coefficients 
and study the general form of the asymptotic flux scalar potential and vacuum conditions by 
considering all possible sl(2)-representations. This 
more abstract approach can be viewed as an avenue to study general aspects of flux vacua and 
eventually provide a classification of possibilities at least in the regime where the sl(2)-approximation is 
valid. Initial steps in this program have been carried out for two-moduli Calabi-Yau fourfolds in \cite{Grimm:2019ixq}.  
Independent of whether one uses the sl(2)-approximation concretely for specific examples or abstractly in a classification, 
we stress that with its help the search for flux vacua is turned into a rather simple algebraic problem. 
It can therefore be viewed as providing the computationally ideal starting point when
looking for vacua of the fully corrected potential.


In order to make use of any results obtained in the sl(2)-approximation, it is crucial to show how closely it approximates 
the full answer. In particular, the second approximation step, the nilpotent orbit approximation, will differ from the 
sl(2)-approximation by subleading polynomial corrections. The presence of these corrections 
complicates the field dependence of the Hodge star  significantly and the search for vacua becomes much more involved
and quickly computationally intractable. We show by studying a number of explicit Calabi-Yau threefold examples, that 
the sl(2)-approximation actually provides a rather good approximation, even for a mild hierarchy among the moduli. 
We show this not only for a large complex-structure regime, but also at so-called conifold-large complex structure 
boundaries that are not straightforwardly 
accessible via large complex-structure/large volume mirror symmetry. The periods of the latter setting 
have been derived in \cite{Blumenhagen:2020ire,Demirtas:2020ffz} and we will see explicitly that the general sl(2)-approximation can be  
evaluated from this information. Our findings will support the claim that the successive approximation scheme 
is powerful not only in specific asymptotic regimes, but rather provides a general systematics 
 in all asymptotic regimes in Type IIB  flux compactifications. 
 
 In the final part of this work we show that our strategy is equally applicable to Calabi-Yau fourfolds used in F-theory flux compactifications. 
We hereby focus on discussing the large complex-structure regime, for which the necessary data that determines the sl(2)-approximation 
can be given in terms of the intersection numbers and Chern classes of the mirror Calabi-Yau fourfold. In order to provide an example computation we 
discuss an explicit Calabi-Yau fourfold that realizes the so-called linear scenario recently proposed in \cite{Marchesano:2021gyv}.\footnote{A related Type IIA version of such 
a scenario has been first proposed in \cite{Palti:2008mg}.} We show that this scenario admits a flat direction in the sl(2)-approximation 
that is subsequently lifted in the nilpotent orbit approximation. Furthermore, we will argue that this does not necessarily imply that 
the tadpole conjecture of \cite{Bena:2020xrh} is violated by adapting a strategy recently suggested in \cite{Plauschinn:2021hkp}. The conjecture claims that in high-dimensional 
moduli spaces not all fields can be stabilized by fluxes without overshooting the tadpole bound. If true, it would have far reaching 
consequences for string phenomenology. The desire to provide evidence for this conjecture, or to disprove it, can be viewed 
as another motivation for implementing a systematic approximation scheme. Remarkably, our constructions can be carried out 
for examples with many moduli without much effort and therefore give an exciting opportunity to explore moduli stabilization 
on higher-dimensional moduli spaces \cite{toappear}. 


This paper is organized as follows. In section \ref{Mod-stab-rev} we briefly recall some basics about 
Type IIB orientifold compactifications, the conditions on flux vacua, and the form of the Hodge star as a function of the 
complex-structure moduli. We give a detailed introduction to the sl(2)-approximation and its derivation 
in section \ref{sec_type_ii_boundary}. The idea is to first collect some intuitive ideas how to see the emergence of an 
sl(2) and thereafter delve in the technical details of the general construction. For concreteness we 
will also exemplify the construction on one explicit example. In section \ref{sec-mod-stab} we then introduce 
the moduli stabilization scheme with the successive approximation steps. We show in a number of 
examples how close the vacua determined in the sl(2)-approximation are to the vacua obtained with 
Hodge star that has all polynomial corrections. Finally, in section \ref{F-theory} we extend the discussion 
to Calabi-Yau fourfolds and F-theory. For simplicity, in this case we only discuss the large complex-structure 
regime in detail. We determine the sl(2)-approximation for a concrete fourfold example and 
show how moduli can be stabilized using the linear scenario of \cite{Marchesano:2021gyv}. This will allow us to comment 
on the compatibility of this scenario with the tadpole conjecture. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Moduli stabilization in the asymptotic regime}\label{sec-mod-stab}
In this section we explain how the sl(2)-approximation can be used as a first step for finding flux vacua. We begin with an overview of the various degrees of approximation in section \ref{ssec:scheme}. Using this scheme we then stabilize moduli for three different examples in complex-structure moduli space in sections \ref{ssec:LCS2}, \ref{ssec:LCS3} and \ref{ssec:coniLCS}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{An approximation scheme for finding flux vacua}\label{ssec:scheme}
In general, it is a rather difficult problem to stabilize moduli in flux compactifications, since the Hodge star operator in the extremization conditions \eqref{eom_003} depends in an intricate way on the underlying complex-structure moduli. In this work we propose to address this problem by approximating the moduli dependence of the scalar potential in three steps as
\tikzstyle{block} = [draw,, rectangle, 
    minimum height=3em, minimum width=2em, align=center]
\begin{equation}
\begin{tikzpicture}[baseline = -0.4ex]
\node[block, text width=4.2cm] (a) at (0,0) {(1) sl(2)-approximation};
\node[block, text width=3.5cm] (b) at (5,0) {(2) Nilpotent orbit approximation};
\node[block, text width=4.5cm] (c) at (10,0) {(3) Full series of \\
exponential corrections };

\draw [ thick, ->] (a) -- (b);
\draw [ thick, ->] (b) -- (c);
\end{tikzpicture}
\end{equation}
By using the sl(2)-approximation as a first step, we break the behavior of the scalar potential down into polynomial terms in the complex-structure moduli. This allows us to solve the relevant extremization conditions for the vevs of the moduli straightforwardly. Subsequently, we can include corrections to this polynomial behavior by switching to the nilpotent orbit approximation. Roughly speaking, this amounts to dropping all exponential corrections in the scalar potential,\footnote{We should stress that one has to be careful where these exponential corrections are dropped. While we can drop corrections at these orders in the scalar potential, essential exponential corrections have to be included in its defining K\"ahler potential and flux superpotential. These terms are required to be present for consistency of the period vector following the discussion of \eqref{Pi-exp2} (see also \cite{Bastian:2021eom, Bastian:2021hpc} for a more detailed explanation).} but including corrections to the simple polynomial terms of the sl(2)-approximation, yielding algebraic equations in the moduli. Taking the flux vacua found in the sl(2)-approximation as input, we then iterate a numerical program to extremize the scalar potential in the nilpotent orbit approximation. Finally, one can include exponentially small terms in the saxions in the scalar potential. In this work we aim to stabilize all moduli at the level of the nilpotent orbit, but in principle one could use these corrections to lift flat directions in the first two steps. 


\subsubsection*{Sl(2)-approximation}
As a starting point, we study the extremization conditions for flux vacua in the sl(2)-ap\-prox\-i\-ma\-tion \eqref{strict-regime} for the saxions. In section \ref{sec_type_ii_boundary} we explained how the Hodge star in this regime can be approximated by the operator $C_{\rm sl(2)}$ given by \eqref{boundarystar}.  By writing the self-duality condition \eqref{eom_001} with $C_{\rm sl(2)}$ we obtain as extremization condition
\begin{equation}\label{self_dual}
C_{\rm sl(2)}(x,y) \ G_3
= i G_3 \, .
\end{equation}
This approximation drastically simplifies how the Hodge star operator depends on the moduli. For the axions the dependence enters only through factors of $e^{- x^k N_k^-} $. It is therefore useful to absorb these factors into $G_3$ by defining flux axion polynomials
\begin{equation}\label{axion_polynomials}
\rho_{\rm sl(2)}(x) \equiv  e^{- x^k N_k^-} G_3  \, .
\end{equation}
Note that $\rho_{\rm sl(2)}$ is invariant under monodromy transformations $x^i \to x^i +1$ when we shift the fluxes according to $G_3 \to e^{N_i^-} G_3$.

For the saxions we can make the dependence explicit by decomposing into eigenspaces of the weight operators $N_i^0$ of the $\mathfrak{sl}(2, \mathbb{R})$-triples. By applying this decomposition for $\rho_{\rm sl(2)}$ we obtain
\begin{equation}\label{rho_sl2}
\qquad \rho_{\rm sl(2)}(x^i)  = \sum_{\ell \in \cE}  \rho_\ell (x^i)\, , \qquad N_i^0 \rho_\ell(x^i) = \ell_i \rho_\ell(x^i)\, ,
\end{equation}
where $\ell = (\ell_1, \ldots , \ell_n)$, and $\cE$ denotes the index set that specifies which values the $\ell_i$ can take.  Generally one has bounds $-d \leq \ell_i \leq d$, with $d$ the complex dimension of the underlying Calabi-Yau manifold, which here is $d=3$. This decomposition \eqref{rho_sl2} allows us to write out the self-duality condition \eqref{self_dual} in terms of the sl(2)-approximated Hodge star \eqref{boundarystar} componentwise as
\begin{equation}\label{self_dual_sl2}
y_1^{\ell_1} \cdots y_n^{\ell_n} \, C_\infty \, \rho_\ell (x^i) =     \rho_{-\ell} (x^i) \, , \qquad \ell \in \cE \, ,
\end{equation}
where $C_\infty$ is the boundary Hodge star operator independent of the limiting coordinates.\footnote{The operator \eqref{Cinfty} is also constructed as a product of the sl(2)-approximation. It can be understood as a Hodge star operator attached to the boundary for the Hodge structure \eqref{Fpinfty} arising in the asymptotic limit.} With \eqref{self_dual_sl2} we now have obtained a simple set of polynomial equations that one can solve straightforwardly.


\subsubsection*{Nilpotent orbit approximation}
For the next step in our approximation scheme we proceed to the nilpotent orbit. Recall that this approximation amounts to dropping some exponential terms in the $(3,0)$-form periods. In order to identify the essential corrections which remain one has to use \eqref{nilp-form} and \eqref{Fp0}. In the end, this yields a set of vector spaces $H^{p,q}_{\rm nil} $ that can be spanned by a basis valued polynomially in the coordinates $x^i, y^i$. Generally speaking, the corresponding Hodge star operator $C_{\rm nil}$ then depends on these coordinates through algebraic functions, in contrast to more general transcendental functions when exponential corrections are included. On the other hand, in comparison to the sl(2)-approximation one finds that $C_{\rm nil}$ contains series of corrections to $C_{\rm sl(2)}$ when expanding in $y_1/y_2, \ldots, y_{n-1}/y_n, 1/y_n \ll 1$. For now, let us simply state the self-duality condition \eqref{eom_001} at the level of the nilpotent orbit as
\begin{equation}\label{self_dual_nil}
C_{\rm nil} \, G_3 = i G_3\, .
\end{equation}
Next, we write out the dependence of $C_{\rm nil}$ on the coordinates in a similar manner as we did for the sl(2)-approximation. The dependence on the axions again factorizes as
\begin{equation}
C_{\rm nil} (x^i, y^i)= e^{x^k N_k} \, \hat{C}_{\rm nil} (y^i)\,  e^{-x^k N_k} \, , \qquad \hat{C}_{\rm nil}  (y^i)= C_{\rm nil}(0, y^i) \, ,
\end{equation}
where here the log-monodromy matrices $N_i$ appear instead of the lowering operators $N_i^-$ of the $\mathfrak{sl}(2,\mathbb{R})$-triples in \eqref{boundarystar}. In analogy to \eqref{axion_polynomials} we then absorb the axion dependence into flux axion polynomials as
\begin{equation}
\rho_{\rm nil} (x^i) = e^{-x^k N_k} G_3\, ,
\end{equation}
which are invariant under monodromy transformations $x^i \to x^i + 1$ if we redefine the fluxes according to $G_3 \to e^{N_i}G_3$. The dependence of $\hat{C}_{\rm nil}$ on the saxions $y^i$ is considerably more complicated than that of the sl(2)-approximated Hodge star operator $C_{\rm sl(2)}$, so we do not write this out further.\footnote{A systematic approach to incorporate these corrections in $y_1/y_2, \ldots, y_{n-1}/y_n, 1/y_n $ to the Hodge star operator was put forward in the holographic perspective of \cite{Grimm:2020cda, Grimm:2021ikg}.} The self-duality condition \eqref{self_dual_nil} can then be rewritten as
\begin{equation}\label{self_dual_nil_expanded}
\hat{C}_{\rm nil}(y^i)\,  \rho_{\rm nil}(x^i) = i \rho_{\rm nil}(x^i)\, .
\end{equation}
This extremization condition can be expanded in any basis of choice for the fluxes by writing out $\rho_{\rm nil}$ componentwise, yielding a system of algebraic equations in the moduli. Our approach in this work is to take solutions of \eqref{self_dual_sl2} as input, and then slowly vary the moduli vevs to find a solution to \eqref{self_dual_nil_expanded}.

\subsubsection*{Exponential corrections}
As a final remark, let us comment on the importance of exponential corrections in the saxions. Following the discussion of \eqref{Pi-exp2} based on \cite{Bastian:2021eom, Bastian:2021hpc}, we can divide the set of exponential corrections into terms that are essential in the period vector and those that are not. The former are included in the nilpotent orbit approximation, while the latter represent subleading corrections.
\begin{itemize}
\item \textit{Essential exponential corrections.} These corrections have to be included in the K\"ahler potential and superpotential when deriving the scalar potential from \eqref{pot_04} in the nilpotent orbit approximation. They give contributions to the polynomial part of the scalar potential, which arise due to non-trivial cancelations with the inverse K\"ahler metric. One is thus allowed to drop exponential terms in the saxions only once the scalar potential has been computed. In particular, we want to point out that these corrections therefore have to be included in the F-term  conditions $D_I W=0$, while in the self-duality condition \eqref{eom_001} exponential terms can be ignored. %This follows from the fact that the scalar potential can be written in terms of the Hodge star operator, so the polynomial part of the self-duality condition corresponds directly to the polynomial part of the scalar potential. 
The fact that the self-duality condition turns moduli stabilization manifestly into an algebraic problem is the reason we prefer to work in this paper with those extremization conditions over the vanishing F-terms constraints.


\item \textit{Non-essential exponential corrections.} These terms in the periods can only produce exponential corrections in the scalar potential.  They are relevant when the nilpotent orbit approximation does not yet suffice to stabilize all moduli, in which case one can use them to lift the remaining flat directions by means of e.g.~racetrack potentials. In this work we stabilize all moduli via \eqref{self_dual_nil_expanded} at the level of the nilpotent orbit, so these corrections can be ignored as long as the saxions take sufficiently large values.

\end{itemize}





\subsection{Large complex-structure limit for $h^{2,1} = 2$}\label{ssec:LCS2}


Let us consider the example discussed in section~\ref{sec_aht_example}. 
We recall the triple intersection numbers of the mirror threefold  from 
\eqref{data_ex_001} as 
\begin{equation}
\kappa_{122}  = 4\, , \hspace{40pt} \kappa_{222} = 8\, ,
\end{equation}
which specify the  K\"ahler metric in the complex-structure sector 
via the prepotential \eqref{data_ex_prepot}. The sl(2)-approximated 
Hodge-star operator in the regime
 $y^1 \gg y^2 \gg 1$
has been shown in \eqref{data_ex_csl2},
where we note that the prepotential contains more detailed information 
about the moduli-space geometry 
than the sl(2)-approximation. In order to 
compare these two approaches, we define the relative difference 
\eq{
\label{diff_01}
  \Delta = \frac{|| \phi^{\rm nil} - \phi^{\rm sl(2)}||}{|| \phi^{\rm nil}||} \,,
}
where $\phi=(y^i,x^i,s,c)$ and where for simplicity we used the Euclidean norm.
To illustrate this point, let us give an explicit example:
\eq{
  \renewcommand{\arraystretch}{1.2}
  \arraycolsep10pt
  \begin{array}{||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||}
  \hline\hline
  \multicolumn{3}{||c||}{\mbox{fluxes}}
  &
  \multicolumn{3}{c||}{\mbox{sl(2)-approximation}}  
  &
  \multicolumn{3}{c||}{\mbox{large complex structure}}  
  \\ \hline
  h^I &=& (0,0,1) 
  & y^i &=& (9.72,2.79) 
  & y^i &=& (7.85,2.79)   
  \\
  h_I &=& (-162,0,0) 
  & x^i &=& (0.00,0.00) 
  & x^i &=& (0.00,0.00)   
  \\
  f^I &=& (1,0,0) 
  &  s &=& 0.93
  &  s &=& 0.93  
  \\
  f_I &=& (0,1,37) 
  & c &=& 0.00
  & c &=& 0.00  
  \\
  \hline
  N_{\rm flux}&=&-199 & \multicolumn{6}{c||}{\Delta=0.22}
  \\
  \hline\hline
  \end{array}
}
The choice of $H_3$ and $F_3$ fluxes together with their tadpole contribution (c.f.~ equation \eqref{tad_01})
is shown in the first column, in the second column we show the location of the minimum 
in the sl(2)-approximation, and in the third column the location of the minimum 
determined using the full prepotential at large complex structure is shown.
These two loci agree reasonably-well even for the small hierarchy of three, and their relative 
difference $\Delta$ is $22\%$. 


Next, we want to investigate how well the sl(2)-approximation to the Hodge-star operator 
agrees with the large complex-structure result depending on the hierarchy of the 
saxions. We implement the hierarchy through a parameter $\lambda$ as follows
\eq{\label{scaling_two_moduli}
  y^1=\lambda^2\,, \hspace{40pt}
  y^2=\lambda\,, 
}  
and for larger  $\lambda$ we expect a better agreement between the two approaches. 
We have considered three different families of fluxes characterized by 
different initial choices for $h^I$, $f^I$ and the axions $x^i$. 
The dependence of the relative difference $\Delta$ on the hierarchy parameter $\lambda$ 
is shown  in figure~\ref{fig_lcs2_01}, and
in figure~\ref{fig_lcs2_02} we shown the dependence of the (absolute value) of the tadpole
contribution $N_{\rm flux}$ on $\lambda$. 
We  make the following observations:
\begin{itemize}

\item As it is expected, for a large hierarchy $\lambda$ the sl(2)-approximation 
agrees better with the large complex-structure result. Somewhat unexpected 
is however how quickly a reasonable agreement is achieved, for instance, for a 
hierarchy of $\lambda=6$ the two approaches agree up to a difference of $15\%$. 

\item Furthermore, it is also expected that when approaching the boundary
in moduli space the tadpole contribution increases, however, the rate 
with which the tadpole increases is higher than naively expected.
For the family corresponding to the green curve in figures~\ref{plot_lcs_all}
the tadpole dependence can be fitted as
\eq{
  N_{\rm flux} = 8.27\, \lambda^{3.99}+34.69 \,,
}
which is in good agreement with the data for $\lambda\geq 2$. Thus, for 
these examples, when approaching the large complex-structure limit the tadpole
contribution increases rapidly. The scaling in $\lambda$ of the tadpole can also be understood from the weights of the fluxes under the $\mathfrak{sl}(2)$-triples. The heaviest charge is $(1,0,0,0,0,0)$ with weights $(\ell_1,\ell_2)=(1,2)$ under $N^0_1,N^0_2$. Using \eqref{boundarystar} for the asymptotic behavior of the Hodge star and plugging in \eqref{scaling_two_moduli} for the saxions we find that
\begin{equation}
N_{\rm flux} \sim (y^1)^{\ell_1} (y^2)^{\ell_2} = \lambda^4\, .
\end{equation}
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\vspace*{15pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot05_lcs2_1.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-205,122){\footnotesize$\Delta$}
\end{picture}
\caption{Dependence of $\Delta$ on $\lambda$.\label{fig_lcs2_01}}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot06_lcs2_2.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-223,117){\footnotesize$N_{\rm flux}$}
\end{picture}
\caption{Log-dependence of $N_{\rm flux}$ on $\lambda$.\label{fig_lcs2_02}}
\end{subfigure}
\caption{Large complex-structure limit for $h^{2,1}=2$: 
dependence of the relative difference $\Delta$ and of the tadpole contribution 
$N_{\rm flux}$ on the hierarchy parameter $\lambda$. The plots show three different families, 
which all show a similar behaviour.\label{plot_lcs2_all}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Large complex-structure limit for $h^{2,1} = 3$}\label{ssec:LCS3}


As a second  example we consider the large complex-structure limit in the case $h^{2,1}=3$, for which the 
prepotential $\mathcal F$ 
appearing in \eqref{pm} is cubic
\eq{
  \label{prepot}
  \mathcal F = -\frac{1}{3!} \frac{\kappa_{ijk} X^i X^j X^k}{X^0} \,, 
}
with $ t^i= x^i+i\op y^i=\frac{X^i}{X^0}$.
For our specific model we chose  the following non-trivial triple intersection numbers
\eq{
  \kappa_{123} =3 \,, \qquad
  \kappa_{133}=4 \,,\qquad
  \kappa_{233}=4\,,\qquad
  \kappa_{333}=5\,,
}
and the the corresponding K\"ahler metric in the complex-structure sector is well-defined inside the K\"ahler 
cone characterized by $\mbox{Im}\op t^i = y^i>0$.

As our sl(2)-approximation for this example we consider the regime $y^1 \gg y^2 \gg y^3 \gg 1$. Using the algorithm laid out in \ref{sec_tech_details}, we construct the sl(2)-approximated Hodge star \eqref{boundarystar}. Let us give the relevant building blocks here. The $\mathfrak{sl}(2)$-triples are given by
\begin{equation}
\begin{aligned}
N_1^- &=\scalebox{0.75}{$  \left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & -3 & 0 & 0 & 0 & 0 \\
 0 & 0 & -3 & -4 & 0 & 0 & 0 & 0 \\
\end{array}
\right)$}\, ,  & N^0_1 &= \scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & -\frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{4}{3} & 0 & -1 \\
\end{array}
\right)$} \,,\\
N_2^- &= \scalebox{0.75}{$  \left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\
 0 & 0 & 0 & -3 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -3 & 0 & -4 & 0 & 0 & 0 & 0 \\
\end{array}
\right)$} \,, &N^0_2 &=\scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & -1 & -\frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & \frac{4}{3} & -1 \\
\end{array}
\right)$} \,,\\
N_3^- &= \scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -\frac{2}{3} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -\frac{2}{3} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{2}{3} & \frac{2}{3} & -1 \\
 0 & 0 & -3 & -2 & 0 & 0 & 0 & 0 \\
 0 & -3 & 0 & -2 & 0 & 0 & 0 & 0 \\
 0 & -2 & -2 & -\frac{8}{3} & 0 & 0 & 0 & 0 \\
\end{array}
\right)$}\, , \hspace{30pt}&N^0_3 &= \scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & \frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & \frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\
 0 & 0 & 0 & 0 & 0 & -\frac{4}{3} & -\frac{4}{3} & 1 \\
\end{array}
\right)$} \,, \\
\end{aligned}
\end{equation}
and the boundary Hodge star by
\begin{equation}
C_\infty = \scalebox{0.85}{$  \left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & \frac{1}{3} & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{13}{27} & \frac{4}{27} & -\frac{2}{9} \\
 0 & 0 & 0 & 0 & 0 & \frac{4}{27} & \frac{13}{27} & -\frac{2}{9} \\
 0 & 0 & 0 & 0 & 0 & -\frac{2}{9} & -\frac{2}{9} & \frac{1}{3} \\
 -3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -3 & 0 & -2 & 0 & 0 & 0 & 0 \\
 0 & 0 & -3 & -2 & 0 & 0 & 0 & 0 \\
 0 & -2 & -2 & -\frac{17}{3} & 0 & 0 & 0 & 0 \\
\end{array}
\right) $} \, .
\end{equation}
Let us now again compare the sl(2)-approximation with the full prepotential at large complex structure, 
and display the following explicit example:
\eq{
  \renewcommand{\arraystretch}{1.2}
  \arraycolsep10pt
  \begin{array}{||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||}
  \hline\hline
  \multicolumn{3}{||c||}{\mbox{fluxes}}
  &
  \multicolumn{3}{c||}{\mbox{sl(2)-approximation}}  
  &
  \multicolumn{3}{c||}{\mbox{large complex structure}}  
  \\ \hline
  h^I &=& (0,0,0,1) 
  & y^i &=& (8.01,4.01,2.00) 
  & y^i &=& (6.39,2.69,2.18)   
  \\
  h_I &=& (-192,0,0,0) 
  & x^i &=& (0.00,0.00,0.00) 
  & x^i &=& (0.00,0.00,0.00)   
  \\
  f^I &=& (1,0,0,0) 
  &  s &=& 1.00
  &  s &=& 1.08  
  \\
  f_I &=& (0,2,8,55) 
  & c &=& 0.00
  & c &=& 0.00  
  \\
  \hline
  N&=&-247 & \multicolumn{6}{c||}{\Delta=0.13}
  \\
  \hline\hline
  \end{array}
}
Similarly as above, the choice of $H_3$ and $F_3$ fluxes 
is shown in the first column, in the second column we show the minimum 
in the sl(2)-approximation, and the third column contains the location of the minimum 
using the full prepotential.
These  loci agree reasonably-well even for the small hierarchy of two, and their relative 
difference $\Delta$ is $13\%$. 


Next, we investigate how well the sl(2)-approximation to the Hodge-star operator 
agrees with the large complex-structure result depending on the hierarchy of the 
saxions. We implement the hierarchy through as follows
\eq{\label{scaling_three_moduli}
  y^1=\lambda^3\,, \hspace{40pt}
  y^2=\lambda^2\,, \hspace{40pt}
  y^3=\lambda\,, 
}  
and for larger  $\lambda$ we expect a better agreement between the two approaches. 
We have again considered three different families of fluxes characterized by 
different initial choices for $h^I$, $f^I$ and the axions $x^i$. 
The dependence of the relative difference $\Delta$ on the hierarchy parameter $\lambda$ 
is shown  in figure~\ref{fig_lcs_01}, and
in figure~\ref{fig_lcs_02} we shown the dependence of the (absolute value) of the tadpole
contribution $N_{\rm flux}$ on $\lambda$. 
We  make the following observations:
\begin{itemize}

\item For a large hierarchy $\lambda$ the sl(2)-approximation 
agrees well with the large complex-structure result. For a 
hierarchy of $\lambda=4$ the two approaches agree up to a difference of $15\%$. 

\item When approaching the boundary
in moduli space the tadpole contribution increases,
and for the family corresponding to the green curve in figures~\ref{plot_lcs_all}
the tadpole dependence can be fitted as
\eq{
  N_{\rm flux} = 3.21\, \lambda^{5.97}+351.16 \,,
}
which is in good agreement with the data for $\lambda\geq 3$. Again we can understand this scaling from the weights of the fluxes under the $\mathfrak{sl}(2)$-triples. The heaviest charge $(1,0,0,0,0,0)$ has weights $\ell_1=\ell_2=\ell_3=1$ under the grading operators $H_i$. Using \eqref{boundarystar} for the asymptotic behavior of the Hodge star and plugging in \eqref{scaling_three_moduli} for the saxions we find that
\begin{equation}
N_{\rm flux} \sim (y^1)^{\ell_1} (y^2)^{\ell_2} (y^3)^{\ell_3} = \lambda^6\, .
\end{equation}

\end{itemize}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\vspace*{15pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot01_lcs_1.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-205,122){\footnotesize$\Delta$}
\end{picture}
\caption{Dependence of $\Delta$ on $\lambda$.\label{fig_lcs_01}}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot02_lcs_2.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-223,117){\footnotesize$N_{\rm flux}$}
\end{picture}
\caption{Log-dependence of $N_{\rm flux}$ on $\lambda$.\label{fig_lcs_02}}
\end{subfigure}
\caption{Large complex-structure limit: dependence of the relative difference $\Delta$ and of the tadpole contribution 
$N_{\rm flux}$ on the hierarchy parameter $\lambda$. The plots show three different families, 
which all show a similar behaviour. Note that in \ref{fig_lcs_02} the green and blue 
line are almost overlapping.\label{plot_lcs_all}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Conifold--large complex-structure limit for $h^{2,1} = 3$}\label{ssec:coniLCS}


As a third example we consider a combined conifold and large complex-structure limit. 
We choose  $h^{2,1}=3$, and send one saxion to a conifold locus in moduli 
space and the remaining two saxions to the large complex-structure point. 
This example has been considered before in \cite{Blumenhagen:2020ire}, but here we neglect the 
instanton contributions to the prepotential. In particular, for our purposes it
is sufficient to consider the following  prepotential  
\eq{
\label{prepot_002}
  \mathcal F =  -\frac{1}{3!} \frac{\kappa_{ijk} X^i X^j X^k}{X^0}  + \frac{1}{2}\op a_{ij} \op X^i X^j + b_i\op X^i X^0 
  + c\op \bigl(X^0\bigr)^2 - \frac{1}{2\pi \op i} \bigl(X^3\bigr)^2 \log\left[ \frac{X^3}{X^0} \right] ,
}
where $i,j,k,=1,\ldots,3$. The non-trivial triple intersection numbers $\kappa_{ijk}$ and 
 constants $a_{ij}$ and $b_i$ are given by
\eq{
  \arraycolsep2pt
  \begin{array}{lcl}
  \kappa_{111} &=& 8\,, \\
  \kappa_{112} &=& 2\,, \\
  \kappa_{113} &=& 4\,, \\
  \kappa_{123} &=& 1\,, \\
  \kappa_{133} &=& 2\,, 
  \end{array}
  \hspace{40pt}
  a_{33} = \textstyle{ \frac{1}{2} + \frac{3-2\log[2\pi]}{2\pi\op i}\,,}
  \hspace{40pt}
  \begin{array}{lcl}
  b_{1} &=& \frac{23}{6}\,, \\
  b_{2} &=& 1\,, \\
  b_{3} &=& \frac{23}{12}\,.
  \end{array}
}
The constant $c$ can be set to zero for the limit we are interested in for simplicity. After computing 
the periods $\partial_I \mathcal F$ and the matrix $\partial_I\partial_J\mathcal F$, we 
set $t^i = X^i/X^0$ and $X^0=1$, and we 
perform a further field redefinition of the form 
\eq{
  t^1 \to \tilde t^1  \,,\qquad
  t^2 \to \tilde t^2+ 4\op \tilde t^3  \,,\qquad
  t^3 \to e^{2\pi \op i\op \tilde t^3} \,,
}
where the tildes will be omitted in the following. 
The domain of our coordinates is then specified by $\mbox{Im}\op t^i = y^i>0$. 

Let us now consider the sl(2)-approximation in the regime $y^3 \gg y^2 \gg y^1 \gg 1$. Using the periods following from the prepotential \eqref{prepot_002} and the algorithm of section \ref{sec_tech_details} we construct the sl(2)-approximated Hodge star \eqref{boundarystar}. The relevant building blocks are the $\mathfrak{sl}(2)$-triples
\begin{equation}
\begin{aligned}
N_1^- &= \scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -\frac{4}{3} & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 5 & 0 & 0 & 0 & 0 & -1 & \frac{4}{3} & 0 \\
 0 & -\frac{16}{3} & -2 & -\frac{8}{3} & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & -1 & 0 & 0 & 0 & 0 \\
 0 & -\frac{8}{3} & -1 & -\frac{4}{3} & 0 & 0 & 0 & 0 \\
\end{array}
\right)$} \,,  \hspace{30pt}&N^0_1 &=\scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & \frac{8}{3} & 2 & \frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & \frac{31}{3} & 4 & \frac{31}{6} & -2 & 0 & 0 & 0 \\
 \frac{31}{3} & 0 & 0 & 0 & 0 & 0 & -\frac{8}{3} & 0 \\
 4 & 0 & 0 & 0 & 0 & 0 & -2 & 0 \\
 \frac{31}{6} & 0 & 0 & 0 & 0 & 0 & -\frac{4}{3} & 0 \\
\end{array}
\right)$}  \,, \\
N_2^- &= \scalebox{0.75}{$\left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & \frac{1}{2} & 0 & 0 & 0 & 0 \\
\end{array}
\right)$}  \,,  &N^0_2 &=\scalebox{0.75}{$\left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & -\frac{1}{2} & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & \frac{1}{2} & 0 & -1 \\
\end{array}
\right)$}\, , \\
N_3^- &= \scalebox{0.75}{$\left(
\begin{array}{cccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 8 & 0 & 0 & 0 & 0 & 0 & -4 & 0 \\
 0 & -8 & 0 & -4 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -4 & 0 & -2 & 0 & 0 & 0 & 0 \\
\end{array}
\right)$}  \,, &N^0_3 &= \scalebox{0.75}{$ \left(
\begin{array}{cccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & \frac{1}{2} & 0 & 0 & 0 & 0 \\
 0 & -\frac{8}{3} & -1 & -\frac{4}{3} & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 5 & 0 & \frac{5}{2} & -1 & 0 & 0 & 0 \\
 5 & 0 & 0 & 0 & 0 & -1 & \frac{8}{3} & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 \\
 \frac{5}{2} & 0 & 0 & 0 & 0 & -\frac{1}{2} & \frac{4}{3} & 0 \\
\end{array}
\right)$}  \,, 
\end{aligned}
\end{equation}
and the boundary Hodge star
\begin{equation}
C_\infty =\scalebox{0.85}{$  \left(
\begin{array}{cccccccc}
 0 & -\frac{23}{24} & -\frac{1}{4} & -\frac{23}{48} & \frac{1}{4} & 0 & 0 & 0 \\
 -\frac{5}{16} & 0 & 0 & \frac{1}{2} & 0 & \frac{5}{8} & -\frac{1}{6} & -1 \\
 -\frac{43}{12} & 0 & 0 & 0 & 0 & -\frac{1}{6} & \frac{38}{9} & 0 \\
 0 & 0 & 0 & -1 & 0 & -1 & 0 & 2 \\
 -\frac{281}{32} & 0 & 0 & 0 & 0 & \frac{5}{16} & \frac{43}{12} & 0 \\
 0 & -\frac{1745}{144} & -\frac{31}{24} & -\frac{1745}{288} & \frac{23}{24} & 0 & 0 & 0 \\
 0 & -\frac{31}{24} & -\frac{1}{2} & -\frac{31}{48} & \frac{1}{4} & 0 & 0 & 0 \\
 0 & -\frac{1745}{288} & -\frac{31}{48} & -\frac{2321}{576} & \frac{23}{48} & -\frac{1}{2} & 0 & 1 \\
\end{array}
\right)$}\, .
\end{equation}
To compare moduli stabilization within the sl(2)-approximation and 
within the conifold-large complex structure limit (coni-LCS), we consider
first the following example
\eq{
  \renewcommand{\arraystretch}{1.2}
  \arraycolsep10pt
  \begin{array}{||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||
  l@{\hspace{2pt}}c@{\hspace{2pt}}l
  ||}
  \hline\hline
  \multicolumn{3}{||c||}{\mbox{fluxes}}
  &
  \multicolumn{3}{c||}{\mbox{sl(2)-approximation}}  
  &
  \multicolumn{3}{c||}{\mbox{coni-LCS}}  
  \\ \hline
  h^I &=& (1,0,0,1) 
  & y^i &=& (1.88,3.78,8.20) 
  & y^i &=& (1.88,2.61,6.92)   
  \\
  h_I &=& (3,-60,1,-30) 
  & x^i &=& (-0.14,-1.27,0.99) 
  & x^i &=& (-0.14,-1.27,1.35)   
  \\
  f^I &=& (0,1,0,0) 
  &  s &=& 1.05
  &  s &=& 1.05  
  \\
  f_I &=& (132,32,0,18) 
  & c &=& 0.07
  & c &=& 0.07  
  \\
  \hline
  N&=&-210 & \multicolumn{6}{c||}{\Delta=0.22}
  \\
  \hline\hline
  \end{array}
}
The hierarchy in the sl(2)-approximation has been chosen as a factor of two, 
the relative difference to the moduli stabilized via the coni-LCS prepotential 
\eqref{prepot_002} for this example is $22\%$. 


Next, we want to study how well the sl(2)-approximation of the Hodge-star operator
captures moduli stabilization via the coni-LCS prepotential. We follow a strategy similar 
to the previous example and implement 
a hierarchy for the saxions through a parameter $\lambda$ as
\eq{\label{scaling_coniLCS}
  y^1=\lambda\,, \hspace{40pt}
  y^2=\lambda^2\,, \hspace{40pt}
  y^3=\lambda^3\,. 
}  
As before, we expect that  for larger  $\lambda$ the agreement between the two approaches
improves. 
We have again considered three different families of fluxes characterized by 
different initial choices for $h^I$, $f^I$ and the axions $x^i$. 
The dependence of the relative difference $\Delta$ on the hierarchy parameter $\lambda$ 
is shown  in figure~\ref{fig_clcs_01}, and
in figure~\ref{fig_clcs_02} we shown the dependence of the (absolute value) of the tadpole
contribution $N_{\rm flux}$ on $\lambda$. 
Our observations agree with the previous example, in particular:
\begin{itemize}

\item we see that even for a small hierarchy of $\lambda=4$ the relative difference between 
the stabilized moduli is only around $10\%$. 


\item The tadpole contribution \eqref{tad_01} grows rapidly with the hierarchy parameter 
$\lambda$. For instance, for the orange curve in figure~\ref{fig_clcs_02} we obtain a fit 
\eq{
  N_{\rm flux} = 4.29\, \lambda^{4.97}+96.71 \,,
}
which is in good agreement with the data for $\lambda\geq3$. Therefore, also for
this example the tadpole contribution increases rapidly when approaching the boundary
in moduli space. Again this scaling is understood from the growth of the Hodge star for the heaviest charge $(1, 0, 0, 0, 0, 23/6, 1, 23/12)$. Using \eqref{boundarystar} we find that
\begin{equation}
N_{\rm flux} \sim (y^1)^{\ell_1} (y^2)^{\ell_2} (y^3)^{\ell_3} = \lambda^5\, ,
\end{equation}
where we used that its weights under the $N^0_i$ are $(\ell_1,\ell_2,\ell_3)=(2,0,1)$, and plugged in the scaling \eqref{scaling_coniLCS} of the saxions in $\lambda$.


\end{itemize}


%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\vspace*{15pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot03_conilcs_1.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-205,122){\footnotesize$\Delta$}
\end{picture}
\caption{Dependence of $\Delta$ on $\lambda$.\label{fig_clcs_01}}
\end{subfigure}
\hspace{20pt}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=200pt]{plot04_conilcs_2.pdf}%
\begin{picture}(0,0)
\put(-6,-9){\footnotesize$\lambda$}
\put(-223,117){\footnotesize$N_{\rm flux}$}
\end{picture}
\caption{Log-dependence of $N_{\rm flux}$ on $\lambda$.\label{fig_clcs_02}}
\end{subfigure}
\caption{Conifold--large complex-structure limit: dependence of the relative difference $\Delta$ and of the tadpole contribution 
$N_{\rm flux}$ on the hierarchy parameter $\lambda$. The plots show three different families, 
which all show a similar behaviour. \label{plot_clcs_all}}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Moduli stabilization in F-theory}\label{F-theory}


We now want to apply the techniques discussed in the above sections to F-theory compactifications on elliptically fibered Calabi-Yau fourfolds. We begin with a brief review of the scalar potential induced by four-form flux, and in section \ref{ssec:lcs} we specialize our discussion to the large complex-structure regime. This  then serves as the starting point for an F-theory example 
which we study in section \ref{ssec:linear} and which has been discussed before in \cite{Marchesano:2021gyv}. For reviews on the subject of F-theory compactifications and its flux vacua we refer the reader to \cite{Denef:2008wq, Weigand:2018rez}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Large complex-structure regime}\label{ssec:lcs}

To make our discussion more explicit, we now  specialize to a particular region in complex-structure moduli space. 
More concretely, we consider the large complex-structure regime  of a Calabi-Yau fourfold $Y_4$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection*{Moduli space geometry}


Using homological mirror symmetry the superpotential can be expressed  in terms of the central charges of B-branes wrapping even-degree cycles of the mirror-fourfold $X_4$, and we refer to the references \cite{Grimm:2009ef,CaboBizet:2014ovf, Gerhardus:2016iot, Cota:2017aal} for a more detailed discussion. Following the conventions of \cite{Marchesano:2021gyv}, we expand the periods of the holomorphic four-form $\Omega$ around the large complex-structure point as
\begin{equation}\label{fourfold_periods}
\Pi = \begin{pmatrix}
1 \\
-t^I \\
\frac{1}{2} \eta_{\mu \nu} \zeta^\nu_{IJ} t^I t^J \\
-\frac{1}{6} \cK_{IJKL} t^J t^K t^L +i K_I^{(3)}\\
\frac{1}{24} \cK_{IJKL} t^I t^J t^K t^L -i K_I^{(3)} t^I
\end{pmatrix},
\end{equation}
where $\cK_{IJKL}$ are the quadruple intersection numbers of $X_4$ and the coefficients $K_I^{(3)}$ arise from integrating the third Chern class. In formulas this reads
\begin{equation}\label{eq:quadruple}
\cK_{IJKL} = D_I \cdot D_J \cdot D_K \cdot D_L\, , \hspace{50pt} K_I^{(3)} = \frac{\zeta(3)}{8\pi^3}\  \int_{X_4} c_3(X_4) \wedge J_I \, ,
\end{equation}
where  $D_I$ denotes a basis of divisor classes for $X_4$ that generate its K\"ahler cone\footnote{We assume the K\"ahler cone to be simplicial, i.e.~the number of generators is equal to $h^{1,1}(X_4)$.} and $J_I \in H^2(X_4, \mathbb{Z})$ denote their Poincar\'e dual two-forms. Under mirror symmetry the $h^{1,1}(X_4)$ K\"ahler moduli $t^i$ of $X_4$ are identified with the $h^{3,1}(Y_4)$ complex-structure moduli of $Y_4$, and the coefficients $K_I^{(3)}$ can be interpreted as perturbative corrections to the periods, similar to the correction involving the Euler characteristic  in the prepotential \eqref{data_ex_prepot} for the threefold case. Furthermore, we introduced a tensor $\zeta^\mu_{IJ}$ to expand all intersections of divisor classes $D_I \cdot D_J$ into a basis of four-cycles $H_\mu$ as
\begin{equation}\label{zeta_tensor}
D_I \cdot D_J = \zeta^\mu_{IJ} H_\mu \, .
\end{equation}
The intersection of two four-cycles $H_\mu \cdot H_\nu$ is  denoted by
\begin{equation}
\eta_{\mu \nu} =  H_\mu \cdot H_\nu\,,
\end{equation} 
and comparing with \eqref{eq:quadruple} leads to the following relation for the intersection numbers 
\begin{equation}
\cK_{IJKL} = \zeta^\mu_{IJ} \op \eta_{\mu\nu} \op \zeta^\nu_{KL} \, .
\end{equation}
The  superpotential  \eqref{fourfold_potentials} shown above can be expressed as $W = G_4 \op\Sigma\op \Pi$, where $\Sigma$
is the matrix coupling the periods to the flux quanta which is  given by
\begin{equation}
\Sigma = \begin{pmatrix}
0 & 0 & 0 & 0 & 1 \\
0 & 0 & 0 & -\delta^I_J & 0 \\
0 & 0 & \eta^{\mu \nu} & 0 & 0 \\
0 & -\delta_I^J & 0 & 0 & 0 \\
1 & 0 & 0 & 0 & 0 \\
\end{pmatrix}.
\end{equation}
Note that we used $I,\mu$ to label the rows and $J,\nu$ for columns. The $G_4$-flux written in these conventions takes the form 
\begin{equation}
G_4 = \left( \, m\,,  \hspace{4pt} m^I \,,  \hspace{4pt} \hat{m}_\mu \,,  \hspace{4pt}  e_I \,, \hspace{4pt}  e\, \right),
\end{equation}
where the flux-quanta are (half-)interger quantized ,
and the contribution of the fluxes to the tadpole cancellation condition is  given by 
\eq{
  N_{\rm flux} = \frac{1}{2} \int_{Y_4} G_4 \wedge G_4 = \frac{1}{2} \op G_4 \Sigma \op G_4\,.
}  
Let us stress that the period vector \eqref{fourfold_periods} is not expanded in an integral basis, which means that special care has to be taken with the quantized fluxes coupling to these periods in the superpotential \eqref{fourfold_potentials}. This quantization was worked out in \cite{Gerhardus:2016iot}, and has been reformulated as a shift of the flux quanta in \cite{Marchesano:2021gyv}. For our purposes having integer-valued fluxes will not be important, so we simply refer to the listed references for more details. 
Finally, it is instructive to decompose the periods in \eqref{fourfold_periods} according to the nilpotent orbit form similar to
the threefold case discussed above. In particular, we can read off the log-monodromy matrices $N_A$ and leading term 
$a_0$ of the periods as
\begin{equation}\label{fourfold_logs}
\Pi = e^{t^I N_I} a_0 \, , \qquad N_A = \begin{pmatrix}
0 & 0& 0 & 0 & 0 \\
-\delta_{AI} & 0 & 0 & 0 & 0 \\
0 & -\eta_{\mu \rho} \zeta^\rho_{AJ} & 0 & 0 & 0 \\
0 & 0 & -\zeta^\nu_{AI} & 0 & 0 \\
0 & 0 & 0 & -\delta_{AJ} & 0 
\end{pmatrix}, \qquad a_0  = \begin{pmatrix}
1 \\
0 \\
0 \\
K^{(3)}_I \\
0
\end{pmatrix}.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Periods for an elliptically fibered mirror}

Let us now specialize to an elliptically fibered mirror fourfold $X_4$, which corresponds to the example considered in the following section. For fourfolds with this fibration structure the topological data of $X_4$ is determined by the base $B_3$, and one can explicitly construct a basis for the four-cycles $H_\mu$ as discussed in \cite{Cota:2017aal}. In the following we work in the conventions of \cite{Marchesano:2021gyv}. 
We start by constructing a basis for the two- and six-cycles of $X_4$ from the base $B_3$. For the generators of the Mori cone of $B_3$ corresponding to two-cycles we write $C'^a$, while the dual four-cycles that generate the K\"ahler cone are denoted by divisors $D'_a$. The index runs as $a = 1, \ldots , h^{1,1}(B_3)$ with $h^{1,1}(B_3) = h^{1,1}(X_4)-1$. Denoting the projection of the fibration by $\pi$ and the divisor class of the section by $E$, we can then generate the Mori cone of $X_4$ by
\begin{equation}
C^0, \qquad C^a = E \cdot \pi^{-1} C'^a \, ,
\end{equation}
where $C^0$ corresponds to the class of the fiber. We generate the K\"ahler cone of $X_4$ by the dual basis of divisor classes
\begin{equation}\label{divisor_basis}
D_0 = E + \pi^* c_1(B_3)\, , \qquad D_a = \pi^* D'_a\, ,
\end{equation}
where $c_1(B_3) = c_1^a D_a'$ denotes the first Chern class of the base $B_3$. We can recover the intersection numbers of $B_3$ from those of $X_4$ as
\begin{equation}
\cK_{abc} = D'_a \cdot D'_b \cdot D'_c = D_0 \cdot D_a \cdot D_b \cdot D_c = \cK_{0abc}\, .
\end{equation}
Having constructed a basis for the two- and six-cycles, let us next consider the four-cycles $H_{\mu}$. We can generate these four-cycles via the divisors $D'_a$ and curves $C'^a$ of $B_3$ as
\begin{equation}\label{fourfold_fourcycles}
H_a = D_0 \cdot \pi^{-1}(D'_a) = D_0 \cdot D_a \, , \qquad H_{\hat{a}} = \pi^{-1} (C'^a)\, , \qquad a,\hat{a} = 1, \ldots , h^{1,1}(B_3) \,,
\end{equation}
where we split $\mu = (a, \hat{a})$. As a final task we construct the tensors $\zeta^\mu_{ij}$ and $\eta_{\mu\nu}$ appearing in the periods \eqref{fourfold_periods}. The tensor $\zeta^\mu_{IJ}$ relating intersections of two-cycles $D_I \cdot D_J$ to the four-cycle basis $H_\mu$ by \eqref{zeta_tensor} is found to be 
\begin{equation}
\zeta_{0b}^a =\delta_{ab}\, , \qquad \zeta^{\hat{a}}_{bc} = \cK_{abc} \, , \qquad \zeta^a_{00} = c_1^a\, ,
\end{equation}
and all other components either vanish or are fixed by symmetry. The intersections $\eta_{\mu \nu}$ between the four-cycles $H_\mu$ are given by
\begin{equation}
 \eta_{ab} = \cK_{abc}c_1^c \, , \qquad \eta_{a\hat{b}} = \delta_{ab} \, , \qquad \eta_{\hat{a} \hat{b}} = 0\, .
 \end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The linear scenario -- construction} \label{ssec:linear}

With the expressions introduced above, we can now discuss a more concrete setting.
We consider the triple fibration $T^2 \to \mathbb{P}^1 \to \mathbb{P}^1 \to \mathbb{P}^1 $ as the mirror fourfold, and 
for  the toric construction  we refer to \cite{Mayr:1996sh}. In \cite{Marchesano:2021gyv} this geometry was used to realize a particular moduli stabilization scheme called the linear scenario. Here we discuss this setup from the perspective of the sl(2)-approximation,
and we comment on the scaling of the corresponding tadpole-contribution of the fluxes.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Moduli space geometry}

The relevant topological data of the above fourfold $X_4$ can be summarized by the following intersection numbers 
\begin{equation}\label{fourfold_volume}
\begin{aligned}
\cK_{ABCD} y^A y^B y^D y^D &= y_L( 32 y_0^3 + 24 y_0 y_1 y_2 +12 y_0 y_2^2 + 24 y_0^2 y_1 + 26 y_0^2 y_2 ) \\
& \ \ \ + 64 y_0^2 y_1 y_2 + 24 y_0 y_1^2 y_2  + 8 y_0 y_2^3
+ 24 y_0 y_1 y_2^2 + 64 y_0^3 y_1 \\
& \ \ \  + 24 y_0^2 y_1^2 + 36 y_0^2 y_2^2 + 72 y_0^3 y_2 + 52 y_0^4 \\
& = 4\op y_L\op \cK_L + f(y^\alpha)\, ,
\end{aligned}
\end{equation}
and by the integrated third Chern class
\begin{equation}
K_A^{(3)}  y^A =-  \frac{\zeta(3)}{8\pi^3} \Big(3136 y^0  + 480 y^L +  960 y^1 + 1080 y^2 \Big)\, ,
\end{equation}
and the base $B_3$ of the elliptic fibration has first Chern class
\begin{equation}
c_1(B_3) =  D_1 + 2D_2\, .
\end{equation}
The divisor $D_0$ corresponds to the zero section of the elliptic fibration as given in  the basis \eqref{divisor_basis}, while $D_L$ corresponds to the class of the Calabi-Yau threefold fiber over $\mathbb{P}^1$. In the last line of \eqref{fourfold_volume} we singled out the terms dependent on the saxion $y^L$  by writing 
\begin{equation}\label{fourfold_functions}
 \cK_L = \sum_{\alpha,\beta,\gamma} \cK_{Labc} y^\alpha y^\beta y^\gamma\, , \qquad f(y^a) = \sum_{\alpha,\beta,\gamma,\delta} \cK_{\alpha\beta\gamma\delta}   y^\alpha y^\beta y^\gamma y^\delta \, ,
\end{equation}
where $f(y^a)$ contains the remaining terms only depending on $y^\alpha=y^0,y^1,y^2$. Let us also note that we sort our complex-structure moduli in the order $(t^0, t^L, t^1 , t^2)$ for the construction of the log-monodromy matrices as described by \eqref{fourfold_logs}, and split the indices as $A=(L, \alpha)$ with $\alpha=0,1,2$. Furthermore, we use the four-cycle basis as described by \eqref{fourfold_fourcycles}, where we let the indices run as $a, \hat{a} = L, 1, 2$.\footnote{Note that this four-cycle basis differs from the one used in \cite{Marchesano:2021gyv}, where another basis was taken using the fibration structure of the threefold fiber rather than the elliptic fiber.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Saxion hierarchies and the sl(2)-approximation}

Let us now introduce particular scalings for the saxions $y_A$. For the linear scenario of \cite{Marchesano:2021gyv} there is a hierarchy $y_L \gg y_\alpha $ which we realize by
\begin{equation}\label{scaling_linear_scenario}
y_L = \lambda^3\, , \hspace{50pt} y_\alpha = \lambda \, \hat{y}_\alpha\, .
\end{equation}
In order to understand this regime from the perspective of the sl(2)-approximation we need to consider a further hierarchy $y_L \gg y_1 \gg y_2 \gg y_0$, which we implement via an additional scaling parameter $\rho$ as
\begin{equation}\label{scaling_linear_sl2}
y_L = \lambda^3 \rho \, , \hspace{50pt} 
y_0 = \lambda  \, , \hspace{50pt}
y_1 = \lambda \rho^2 \, , \hspace{50pt}
y_2 = \lambda \rho\, .
\end{equation}
Setting for instance $\rho = \lambda$ we find scalings $(y_L, y_0,y_1,y_2) = (\lambda^4 , \lambda, \lambda^3, \lambda^2)$ as needed for the hierarchy of the sl(2)-approximation, while for $\rho = 1$ we reduce to a scaling of the form of \eqref{scaling_linear_scenario}. Typically we will keep both the scaling in $\rho$ and $\lambda$ explicit rather than making a choice for $\rho$. We can then use the scaling in $\lambda$ found in the sl(2)-approximation to make statements about the linear scenario. In order to keep the discussion here concise we included the data specifying the sl(2)-approximated Hodge star in appendix \ref{app:linearscenario}. It is, however, instructive to give the eigenspaces of the weight operators $N^{0}_i$, which have been summarized in table \ref{linear_scenario_eigenspaces}.

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\renewcommand*{\arraystretch}{1.8}
\begin{tabular}{| c | c |}
\hline weights  & charges \\ \hline  \hline
$(-1,-3)$ & $(0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 1) $ \\ \hline
$(-1,-1)$ & \begin{minipage}{0.43\textwidth}\centering\vspace*{0.2cm}
$(0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 1, 0, 0, 0, 0)$\\
$ (0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 1, 0, 0)$ \\
$(0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 1, 0 ) $ \vspace*{0.2cm}
\end{minipage} \\ \hline
$(-1,1)$ & \begin{minipage}{0.43\textwidth}\centering\vspace*{0.2cm}
$(0, 0, 0, 0, 0, 0, 1, 0, 0, 0, 0, 0, 0, 0, 0, 0)$ \\
$(0, 0, 0, 0, 0, 0, 0, 1, 0, 0, 0, 0, 0, 0, 0, 0)$ \\
$(0, 0, 0, 0, 0, 0, 0, 0, 1, 0, 0, 0, 0, 0, 0, 0)$ \vspace*{0.2cm}
\end{minipage} \\ \hline
$(-1,3)$ & $( 0, 0, 1, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0)$ \\ \hline
$(1,-3)$ & $(0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 1, 1, 1, \tfrac{1}{2}, 0)$ \\ \hline
$(1,-1)$ & \begin{minipage}{0.43\textwidth}\centering\vspace*{0.2cm}
$(0, 0, 0, 0, 0, 1, 0, 0, -\tfrac{1}{2}, 1, -1, 0, 0, 0, 0, 0)$\\
$(0, 0, 0, 0, 0, 0, 1, 0, 1, -\tfrac{3}{2}, 1, 0, 0, 0, 0, 0)$\\
$(0, 0, 0, 0, 0, 0, 0, 1, -1, 1, 0, 0, 0, 0, 0, 0)$ \vspace*{0.2cm}
\end{minipage} \\ \hline
$(1,1)$ & \begin{minipage}{0.43\textwidth}\centering\vspace*{0.2cm}
$(0, 1, 0, 0, -2, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0)$\\
$(0, 0, 1, 0, -2, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0)$ \\
$(0, 0, 0, 1, -2, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0)$\vspace*{0.2cm}
\end{minipage} \\ \hline
 $(1,3)$ & $(1, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0)$ \\ \hline
\end{tabular}
\caption{\label{linear_scenario_eigenspaces} Eigenspaces of the weight operators given in \eqref{linear_operators_weights}. In order to connect to the scaling of the linear scenario \eqref{scaling_linear_scenario} we grouped the weights $\ell_\alpha$ under $N^0_\alpha$ together as $(\ell_L, \ell_0+\ell_1+\ell_2)$. }
\end{table}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Parametric scaling of the tadpole}


Regarding this model, the aim in  \cite{Marchesano:2021gyv} was to make a flux-choice which keeps the tadpole contribution 
$N_{\rm flux}$ finite
asymptotically. The parametric growth of the tadpole due to a flux is specified by its weights under the $\mathfrak{sl}(2, \mathbb{R})$-triples and we recall that for a charge in the eigenspace  $q \in V_{\ell_1 \ell_2 \ell_3 \ell_4}$ its Hodge norm \eqref{boundarystar} grows as
\begin{equation}
\| q \|^2 \sim y_L^{\ell_L}\op y_0^{\ell_0} \op y_1^{\ell_1}\op y_2^{\ell_2} \, .
\end{equation}
Using the scalings of the saxions shown in \eqref{scaling_linear_sl2}, we find for large $\lambda$ that $3\ell_L+\ell_0+\ell_1+\ell_2 \leq 0$ must hold for our flux quanta. From \eqref{linear_operators_weights} we can compute that $\ell_A = \pm 1$ for all weights, so the fluxes with weights $\ell_L=1$ and $\ell_0+\ell_1+\ell_2 =-1,1,3$ should be turned off. Inspecting table \ref{linear_scenario_eigenspaces} we then find that this corresponds to the flux choice 
\begin{equation}\label{linear_fluxes}
m=0\,,  \qquad m_i = (0,m_L,0,0), \qquad \hat{m}^\mu = (0, \hat{m}^1, \hat{m}^2, \hat{m}^{\hat{L}},0,0)\, , 
\end{equation}
and all other fluxes unconstrained. This matches precisely with the fluxes that were turned off in \cite{Marchesano:2021gyv},  motivated from the sl(2)-approximation.
(Note that we chose a different four-cycle basis as compared to \cite{Marchesano:2021gyv} so the choice of $\hat{m}^\mu $ 
takes a slightly different form.)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection*{Flat directions}

Given the above choice of fluxes, we can now investigate the stabilization of the saxions within various approximation schemes.  
Via the self-duality condition of the $G_4$-flux, the axions are fixed as
as \cite{Marchesano:2021gyv}
\begin{equation}\label{linear_axions}
\begin{aligned}
x^\alpha &= - \frac{\hat{m}^\alpha}{m^L} \, ,  \qquad &x^L &=  - \frac{e}{e_L} - \frac{1}{3 e_L (m^L)^2 } \Big( \cK_{Labc} \hat{m}^a \hat{m}^b \hat{m}^c - 3 e_a \hat{m}^a m^L \Big)\, .
\end{aligned}
\end{equation}
However, for simplicity we  set these axions to zero in the following, that is $x^L=x^0=x^1=x^2=0$, 
which means we impose $e=\hat{m}^1=\hat{m}^2= \hat{m}^{\hat{L}}=0$ on the flux quanta in addition to \eqref{linear_fluxes}.
\begin{itemize}


\item \textit{sl(2)-approximation}: For the specified choice of fluxes \eqref{linear_fluxes} with vanishing axions we find $(1, -3)$ and $(-1, 3)$ as allowed weights for $(\ell_L, \ell_0+\ell_1+\ell_2)$. 
Using the sl(2)-approximated Hodge star \eqref{boundarystar} in the self-duality condition \eqref{fourfold_extremization}, this 
leads to
\begin{equation}
e_L = - \frac{y_0 \op y_1 \op y_2}{2\op y_L} m_L \, , \qquad e_\alpha = 2 e_L\, .
\end{equation}
Notice that the saxions only appear as the combination $y_0 y_1 y_2 / y_L$, so there are three saxionic directions left unconstrained. In particular, when plugging in the scaling of the linear scenario \eqref{scaling_linear_scenario} we see that $\lambda$ drops out completely. We can stabilize these seemingly flat directions by including corrections to the sl(2)-approximation. 


\item \textit{Nilpotent orbit approximation}: We next include the full set of polynomial terms in the periods, in  particular, we investigate the difference between including the corrections $K^{(3)}_i$ or not. The relevant extremization conditions for the saxions now read \cite{Marchesano:2021gyv}
\begin{equation}\label{linear_solve}
\begin{aligned}
e_L &= -\frac{\cK}{6} g_{LL} m^L = \Big( -\frac{ \cK_L}{t_L}+ \frac{ f }{24 t_L^2 }  -\frac{ 
K_L^{(3)} \zeta(3)}{64 \pi^3 t_L}\Big) m^L+ \cO\Big(\frac{1}{\lambda^4}\Big) \, , \\
e_\alpha &= \frac{m^L}{6}  \cK_L \partial_\alpha \Big( \frac{f}{4 \cK_L} \Big) -  \frac{ 9 K^{(3)}_L  \cK_{L\alpha} m^L }{8  \cK_L }+ \cO\Big(\frac{1}{\lambda^2}\Big) \, ,
\end{aligned}
\end{equation}
where $\cK_{L \alpha} = \sum_{\beta, \gamma} \cK_{L \alpha \beta \gamma} y^\beta y^\gamma$. We also specified the order in $\lambda$ at which corrections to these equations enter under the scaling \eqref{scaling_linear_scenario}. Note that only $K^{(3)}_L$ appears here, so it dominates over the other corrections $K^{(3)}_\alpha$ in the expansion in $\lambda$. 
Since it is rather difficult to solve \eqref{linear_solve} explicitly for the saxions, we will instead consider some specific flux quanta $e_L, e_\alpha$ to exemplify that the saxions can indeed be stabilized. 
As flux quanta we take
\begin{equation}
m_L =  623\, , \qquad e_A = (-4698, -3072, -2760, -1566 )\, ,
\end{equation}
for which the saxions \eqref{scaling_linear_scenario} are  stabilized at
\begin{equation}
\lambda = 6 \, , \qquad \hat{y}^\alpha = 1\, .
\end{equation}



\item \textit{Nilpotent orbit approximation without $K^{(3)}_L$}: We also compute the eigenvalues of the mass matrix $K^{ab} \partial_a \partial_b V$ while formally setting $K^{(3)}_L = 0$ and  $K^{(3)}_\alpha = 0$. This yields the canonically-normalized masses
\begin{equation}\label{masses_without}
m^2  = \bigl (
3.4 \cdot 10^{18}, \ 1.7 \cdot 10^{13}, \ 1.7 \cdot 10^{13}, \ 1.7 \cdot 10^{13}, \ 1.6 \cdot 10^{13}, \ 3.8 \cdot 10^{11}, \ 2.7 \cdot 10^{11}, \ 0) \, ,
\end{equation}
and hence for this setting there is one flat direction.

\item \textit{Nilpotent orbit approximation with $K^{(3)}_L$}: We then include the correction $K^{(3)}_L $ but still set $K^{(3)}_\alpha = 0$ and find that the flat direction now acquires a mass
\begin{equation}\label{masses_with}
m^2 = \bigl(3.4 \cdot 10^{18}, \ 1.7 \cdot 10^{13}, \ 1.7 \cdot 10^{13}, \ 1.7 \cdot 10^{13}, \ 1.6 \cdot 10^{13}, \ 3.6 \cdot 10^{11}, \ 2.5 \cdot 10^{11}, \ 2.3 \cdot 10^7 \bigr) ,
\end{equation}
while the other masses are only affected slightly. The now non-zero mass is significantly smaller as compared to the other moduli, since its mass scale is set by the correction $K_L^{(3)}$ rather than the leading polynomial terms.

\end{itemize}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Type IIB2 case}


In order to understand the above observations better, let us reduce the F-theory setting to Type IIB string theory. This brings us to the IIB2 moduli stabilization scheme of \cite{Marchesano:2021gyv}, which was originally considered in \cite{Palti:2008mg}. In order to  match 
the two configurations we set $f=0$ and $K^{(3)}_\alpha = 0$, and identify $K_{L\alpha \beta \gamma}$ with the intersection numbers of the Calabi-Yau threefold and $K^{(3)}_L$ as the Euler characteristic correction. Furthermore, the dilaton $t^L$ is interpreted as the axio-dilaton $\tau$. We will keep the notation of the F-theory setting, and simply drop the terms that are absent in the Type IIB setup, for which the self-duality condition \eqref{linear_solve}  reduces to
\begin{equation}\label{IIB_solve}
\begin{aligned}
e_L & = \Big( -\frac{1}{6} \frac{\cK_L}{y_L}  -\frac{ 
K_L^{(3)} \zeta(3)}{64 \pi^3 y_L}\Big) m^L\, , \qquad &e_\alpha &=  -  \frac{ 9 K^{(3)}_L  \cK_{L\alpha} m^L }{8  \cK_L }\, .
\end{aligned}
\end{equation}
When we drop the correction $K_L^{(3)}$ and plug in the saxion scaling \eqref{scaling_linear_scenario} we see that $\lambda$ cancels out of these equations. However, subsequently including the correction fixes $\lambda$ as
\begin{equation}\label{lambda_vev}
\lambda^3 = \frac{64 \pi ^3}{K_L^{(3)} \zeta(3)} \Big( - \frac{1}{6} \cK_{L\alpha \beta \gamma}\hat{y}^\alpha \hat{y}^\beta \hat{y}^\gamma - \frac{e_L}{m^L}  \Big)\, .
\end{equation}
Thus in the IIB2 scenario the modulus $\lambda$ parametrizes precisely the flat direction we encountered before, which is stabilized by including perturbative corrections. In the general F-theory setup this symmetry was more difficult to spot in \eqref{scaling_linear_scenario} due to the presence of the function $f(\hat{y}^\alpha)$ which alters this parametrization. Nevertheless, by studying the effect of $K_L^{(3)}$ on the masses in \eqref{masses_without} and \eqref{masses_with} we were able to observe this feature.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The linear scenario -- discussion} 

We now want to discuss the linear scenario in view of relations to swampland conjectures, 
to the finiteness theorem and to the tadpole conjecture. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Relations to swampland conjectures and finiteness theorem}
The above hierarchy in the masses of the linear scenario is quite interesting in light of some swampland conjectures. Say we place a cutoff scale between the moduli masses stabilized in \eqref{masses_without} and the field direction stabilized by the $K^{(3)}_L$ effect in \eqref{masses_with}. From the mass hierarchy it then follows that we can integrate out all axion fields (and three saxion fields), while one runaway direction remains. In the IIB2 case this direction is parametrized via the saxionic modulus $\lambda$ by \eqref{scaling_linear_scenario}, while in the more general F-theory setup this parametrization is slightly more involved. Either way, by restricting to this valley of the scalar potential we obtain a pseudomoduli space containing a single saxion field and no axions. In turn, we can send $\lambda \to \infty$, resulting in an infinite distance limit. Generically this path does not lift to a geodesic in the original higher-dimensional moduli space, so this provides us with an interesting class of examples for the Convex Hull Distance Conjecture of \cite{Calderon-Infante:2020dhm}. On the other hand, this infinite distance limit is rather intriguing from the perspective of the Distant Axionic String Conjecture \cite{Lanza:2020qmt, Lanza:2021qsu}. It predicts the emergence of asymptotically tensionless strings coupled to axion fields, but in this effective field theory all axions have already been integrated out due to the cutoff. It would be interesting to return to this puzzle in the near future, and see if a more detailed study of axion strings in the background of such scalar potentials elucidates this matter.

Let us also comment on the linear scenario in the context of the general finiteness theorems for flux vacua satisfying 
the self-duality condition \cite{Grimm:2020cda, Bakker:2021uqw,Grimm:2021vpn}. A first observation is 
that the tadpole $N_{\rm flux} = - e_L m^L$ seems to be independent of the flux $e_\alpha$. However, it is not hard to 
see that $e_\alpha$ cannot be chosen freely and 
there are only finitely many choices allowed in this setting. The second equation in \eqref{IIB_solve} implies that if we 
want to increase $e_\alpha$, we either have to increase $m^L$ or decrease the moduli. In the former case, we immediately 
see that the tadpole grows, while in the latter case we reach a point where our use of the asymptotic results are no longer applicable. 
Furthermore, we check that the possible vevs for the saxions are bounded from above, which is another necessary condition for the finiteness of solutions. 
Inserting the scaling \eqref{scaling_linear_scenario} into the first equation of \eqref{IIB_solve} we see that the $\hat{y}^\alpha$ are bounded from above. Namely, otherwise $e_L$ grows as we increase the volume $\cK_{L\alpha \beta \gamma} \hat{y}^\alpha \hat{y}^\beta \hat{y}^\gamma $, resulting in a diverging tadpole $N_{\rm flux} = - e_L m^L$. Using similar reasoning we find that $\lambda$ is bounded through the condition \eqref{lambda_vev}. 

Finally, let us also have a closer look at the flux vacuum loci themselves. In particular, consider the case $K_L^{(3)}=0$. 
For such geometries the modulus $\lambda$ is unfixed due to the absence of corrections in the nilpotent orbit approximation. 
This means the resulting flux vacua are not point-like, but rather infinite lines stretching to the boundary of moduli space.\footnote{It could be the case that the 
inclusion of exponential corrections stabilizes this flat direction. There are, however, examples where such corrections are absent \cite{Bakker:2021uqw}. 
In that regard it is interesting to point out the work of \cite{Palti:2020qlc}, where the absence of instantons in special cases was related to higher-supersymmetric settings.} 
It is interesting to point out that vacuum loci of this type do not need to be algebraic. This implies that if one aims to describe the structure of all flux vacua one has to 
leave the world of algebraic geometry. Remarkably, a delicate and powerful extension of algebraic geometry that can be use to describe flux vacua is provided by using 
tame topology and o-minimality \cite{Bakker:2021uqw}. The resulting tame form of geometry manifest the notion of finiteness and removes many pathologies that 
are allowed in geometric settings based on ordinary topology. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{Tadpole conjecture I -- without axions}

We now focus on the tadpole contribution of the fluxes and its scaling with the number of 
moduli \cite{Bena:2020xrh,Bena:2021wyr}. For simplicity we restrict our attention to the IIB2 case, 
and our discussion follows closely the line of arguments first presented in \cite{Plauschinn:2021hkp}.
In particular, we will be using statistical data for Calabi-Yau threefolds obtained  in \cite{Demirtas:2018akl}
to show that the linear scenario is, under certain genericity assumptions, compatible with the tadpole conjecture.
Our main argument can then be summarized  as follows:
\begin{itemize}

\item Since we restrict our discussion to the large complex-structure limit and ignore instanton corrections, 
we need to ensure that the latter are sufficiently suppressed. To implement this constraint 
on the mirror-dual side, we require that all holomorphic curves $\cC$ have a volume greater than a 
constant $c$. Similarly we require that all divisors $D$ and the mirror threefold $\tilde Y_3$ itself to have volumes greater than $c$,
and we use these conditions to define the stretched K\"ahler 
cone \cite{Demirtas:2018akl}, i.e.~we consider those $J$ that satisfy 
\beq \label{Kahler-cone}
  \int_C J > c\ , \qquad  \frac{1}{2}\int_D J^2 > c\ , \qquad  \frac{1}{6}\int_{\tilde Y_3} J^3 > c\ . 
\eeq
Note that (after applying mirror-symmetry) the asymptotic regime introduced at the beginning of section \ref{sec_tech_details} lies in the stretched K\"ahler cone with $c=1$. 

\item In \cite{Demirtas:2018akl} the authors analyzed the Kreuzer-Skarke list \cite{Kreuzer:2000xy} 
and determined properties associated with the stretched K\"ahler cone. Via mirror symmetry, these results on the K\"ahler-moduli 
side then translate to the large complex-structure limit we are interested in.

\item  We note that the K\"ahler form $J$ can be expanded in any basis of the second cohomology.  
For example, we can use the generators $\omega_\alpha$ of a simplicial subcone 
as discussed in more detail in \cite{Grimm:2019bey} and 
write $J=y^\alpha\omega_\alpha$. Setting $c=1$ in \eqref{Kahler-cone} then implies $y^\alpha>1$ and we obtain the 
above parametrization of the asymptotic regime. However, in \cite{Demirtas:2018akl} the 
analysis was carried out in a basis naturally arising in the explicit construction of Calabi-Yau threefold examples. Denoting this
basis by $[D_\alpha]$ we expand $J= v^\alpha [D_\alpha]$. We note that the $v^\alpha$ now obey certain non-trivial inequalities 
for $J$ to be an element of the stretched K\"ahler cone \eqref{Kahler-cone}. Clearly, also the intersection numbers $\kappa_{\alpha \beta \gamma} = D_\alpha \cdot D_\beta \cdot D_\gamma$ have to be 
evaluated in this different basis and the statistical statements of \cite{Demirtas:2018akl} concerning their behaviour is generically true in this `special' basis.  



\item Of interest to us are the number of non-zero entries in the triple intersection numbers $\kappa_{\alpha\beta\gamma}$ 
and a measure for how stretched the K\"ahler cone is at large $h^{1,1}$. To associate a number to the latter, we introduce 
the distance $|v| = \sqrt{\sum_a(v^a)^2}$ from the origin of the K\"ahler cone to a K\"ahler form $J= v^a [D_a]$, and 
denote by $d_{\rm min}$ the minimal distance between the origin of the K\"ahler cone and the tip of the stretched K\"ahler cone. 
In  \cite{Demirtas:2018akl}  these have been determined for the Kreuzer-Skarke database and their dependence 
on $h^{1,1}$ have been determined. Under mirror symmetry this dependence translates into\footnote{
When using the basis $\omega_{\alpha}$ to expand the K\"ahler form then the dependence of the quantities in \eqref{rel_9379274}
on $h^{2,1}$ will be different. Since this information is not readily available, we use the basis employed in 
\cite{Demirtas:2018akl}.}
\eq{
  \label{rel_9379274}
   \#(\kappa_{\alpha\beta\gamma}\neq 0) \gtrsim 6.5\op h^{2,1} + 25\,,
   \hspace{40pt}
    d_{\rm min} \simeq 10^{-1.4} \op (h^{2,1})^{2.5}  \,.
}
Furthermore,  for large $h^{2,1}$ the size of the entries of $\kappa_{\alpha\beta\gamma}$ is of order $\mathcal O(10)$ 
which can be inferred from figure 2 of \cite{Demirtas:2018akl}.  For generic situations and in the large $h^{2,1}$ limit 
we then obtain the following rough scaling behavior (see \cite{Plauschinn:2021hkp} for details on the derivation) 
\eq{
  \label{fits_001}
  \cK_L \sim  (h^{2,1})^{-1/2} \op | v |^3 \,,
  \hspace{50pt}
  \cK_{L\alpha} \sim (h^{2,1})^{-1} \op | v  |^2
  \hspace{50pt}
  \cK_L^{(3)} \sim h^{2,1} \,.
}
We included here the quantity $K_L^{(3)}$ which contains the Euler characteristic.
Note that this scaling behaviour matches roughly the statistical analysis presented in \cite{Demirtas:2018akl} for the minimal 
total volume and divisor volumes in the stretched K\"ahler cone when replacing $|v|$ with $d_{\rm min}$. 
  
\end{itemize}
Let us now use \eqref{fits_001} and determine the moduli-dependent expression 
in the second relation in equation \eqref{IIB_solve}. 
For generic situations and for large $h^{2,1}$ we can make the following estimate 
\eq{
  \label{rel_8394}
   \frac{ 9K^{(3)}_L  \cK_{L\alpha}}{8\cK_L } \sim (h^{2,1})^{1/2} \op | v |^{-1} \lesssim (h^{2,1})^{-2} \,,
}
where in the second step we  applied the bound 
 $| v | \geq d_{\rm min}$ and where we ignored numerical factors. 
This scaling can now be used in the self-duality condition  \eqref{IIB_solve}, where the second condition 
together with \eqref{rel_8394} translates to 
\eq{
e_\alpha \lesssim (h^{2,1})^{-2} \op m^L\,.
}
However, 
since the fluxes $e_{\alpha}$ and $m^L$ are integer quantized
it follows that for non-zero $e_{\alpha}$ and $m^L$ the flux $m^L$ has to scale at least as $(h^{2,1})^2$.
For the tadpole contribution this implies 
\eq{
  N_{\rm flux} = - e_L m^L  \sim (h^{2,1})^2 \,,
}
which is in agreement with the tadpole conjecture. 


While this result is non-trivial, let us emphasize that we have used fitted statistical data to make this estimate. 
Some of our steps, most notably \eqref{rel_8394}, are true only approximately and are made under the assumption that 
conspicuous cancellations are absent. 
Comparing \eqref{fits_001} with statistical results on the divisor volumes obtained in \cite{Demirtas:2018akl} shows 
agreement, but ideally we would like to have available results on the minimal value that $\cK_{L}/\cK_{L\alpha} $ can take in the stretched K\"ahler cone directly. 
Moreover, it is conceivable that certain families of compactification spaces exist that show a slightly different scaling behaviour. 
Hence, we do not claim that the IIB2 moduli stabilization scheme of \cite{Marchesano:2021gyv} cannot produce examples 
that violate the tadpole conjecture -- however, under the assumptions stated above the 
scheme of \cite{Marchesano:2021gyv} generically satisfies the tadpole conjecture
(in the case of vanishing axions). 
Note that a similar observation has  been made independently in \cite{Lust:2021xds}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection*{Tadpole conjecture II -- including axions}


We finally want to discuss the case of non-vanishing axions.
Having non-zero fluxes $\hat{m}^\mu$ introduces additional terms, and the modified self-duality equation in F-theory reads
\begin{equation}
m^L e_\alpha -\frac{1}{2} \cK_{L \alpha \beta \gamma} \hat{m}^\beta \hat{m}^\gamma = (m^L)^2 \bigg( \frac{1}{6}  \cK_L \partial_\alpha \Big( \frac{f}{4 \cK_L} \Big)  -  \frac{ 9 K^{(3)}_L  \cK_{L\alpha} }{8  \cK_L } \bigg)\, .
\end{equation} 
For the type IIB limit we set  $f=0$, and together with the first relation in \eqref{IIB_solve} the self-duality condition 
can be expressed as
\eq{
\label{rel_0987}
e_L  = \Big( -\frac{1}{6} \frac{\cK_L}{y_L}  -\frac{ 
K_L^{(3)} \zeta(3)}{64 \pi^3 y_L}\Big) m^L\, , 
\qquad
m^L e_\alpha -\frac{1}{2} \cK_{L \alpha \beta \gamma} \hat{m}^\beta \hat{m}^\gamma = -  \frac{ 9 K^{(3)}_L  \cK_{L\alpha} (m^L)^2 }{8  \cK_L }\,.
}
We now want to repeat our reasoning from above, for which we have to distinguish two cases:
\begin{itemize}


\item We first consider the case in which  the combination 
$m^L e_\alpha -\frac{1}{2} \cK_{L \alpha \beta \gamma} \hat{m}^\beta \hat{m}^\gamma $
appearing in the second relation of \eqref{rel_0987} is generic, in particular, for large $m^L$ this combination 
is a (half-)integer of order $m^L$ (or larger). Using then the scaling \eqref{rel_8394}, we conclude 
again that 
\eq{
  m^L \sim (h^{2,1})^2 
  \hspace{40pt}\Longrightarrow\hspace{40pt}
  N_{\rm flux} \sim (h^{2,1})^2 \,,
}
as in our discussion for vanishing axions. Hence, also in this situation the tadpole conjecture is satisfied. 


\item As a second case we consider a situation where the combination
$m^L e_\alpha -\frac{1}{2} \cK_{L \alpha \beta \gamma} \hat{m}^\beta \hat{m}^\gamma $
is fine-tuned to a non-vanishing $\mathcal O(1)$ half-integer. Here we only need to require 
a linear scaling of $m^L$ with $h^{2,1}$, which leads to 
\eq{
  m^L \sim h^{2,1}
  \hspace{40pt}\Longrightarrow\hspace{40pt}
  N_{\rm flux} \sim h^{2,1} \,.
}
The scaling behaviour of the tadpole conjecture is therefore satisfied also in this non-generic situation. 


\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions}
In this work we have presented a novel strategy for systematically stabilizing complex-structure moduli  in Type IIB and F-theory flux compactifications. For generic regions in field space the underlying scalar potential is known to be a complicated transcendental function of the complex-structure moduli. However, a remarkably universal structure emerges 
when we move towards an asymptotic regime, i.e.~when we approach the boundaries of the moduli space. Motivated by key results from asymptotic Hodge theory, we laid out an approximation scheme to study flux vacua in such settings. This procedure approximates the dependence on the moduli in three steps, which are given by: (1) the sl(2)-approximation, (2) the nilpotent orbit approximation, and (3) the full series of exponential corrections. The first two steps both drop exponential corrections to the scalar potential, therefore yielding a system of algebraic extremization conditions for the moduli. In fact, in the sl(2)-approximation the self-duality condition reduces even further to a simple set of polynomial equations. By iterating through these degrees of approximation and improving the moduli vevs at each step, we turn moduli stabilization into an organized procedure where the complicated dependence on the moduli has been broken down systematically. 

It is important to stress that our approach can be realized in every 
asymptotic regime and generally we find that both approximations (1) and (2) are non-trivial. In particular, determining the nilpotent orbit 
approximation (2) might be familiar for the large complex structure regime, where exponential 
corrections nicely decouple. However, this decoupling does not happen on most other boundaries and dropping exponential corrections becomes a non-trivial 
step that has to be performed when determining the nilpotent orbit. The derivation of the sl(2)-approximation~(1) is non-trivial in essentially all 
asymptotic regions including the large complex structure regime.      
For this reason, in section~\ref{sec_type_ii_boundary} we gave an extensive introduction that explains pedagogically how to construct this sl(2)-approximation step-by-step. Furthermore, in order to exemplify this story, we worked out an explicit two-moduli example in great detail. The goal of this approximation is to derive a representation of sl(2)$^n$ and the boundary Hodge decomposition 
that arise for a $n$-parameter limit in complex-structure moduli space.
In order to do that one has to impose a hierarchy among the complex-structure saxions, and if one restricts attention to this strict asymptotic regime 
corrections proportional to ratios between the saxions can be dropped. The sl(2)$^n$-representation and the boundary Hodge decomposition can then be 
computed algorithmically by iterating through the saxion hierarchies. The resulting data allowed us to introduce an sl(2)-approximated version of the Hodge star 
denoted by $C_{\rm sl(2)}$. It encodes in a simple fashion how 
the Hodge norm behaves in the strict asymptotic regime. Furthermore, the properties of $C_{\rm sl(2)}$ 
allow us to write down polynomial conditions that need to be satisfied for flux vacua in this approximation. 
  

The sl(2)-approximation turns the original very complicated problem of solving the flux vacuum conditions into a tractable 
polynomial task. We explicitly carried out its construction for a number of examples, and showed that the vacua found with this method  resemble the vacua found in the nilpotent orbit approximation rather well --- even if one imposes only a moderate hierarchy of the saxions. 
Raising the hierarchy to an $\mathcal O(10)$-factor we found that the location of vacua in approximation (1) and (2) differ only by few percent. This was true 
in a two-moduli and two three-moduli examples in which we derived the sl(2)-approximation, i.e.~both in the large complex-structure and the conifold-LCS regime. 
Combining these observations with the fact that the approximation (2) and (3) differ only by exponentially suppressed corrections \cite{Schmid}, we thus realize that our proposed 
stabilization scheme gives a favourable numerical approach for finding vacua. It would be very interesting to explore if this gives a novel way to 
perform moduli stabilizations in settings with many moduli and compare the efficiency with direct searches for vacua. We expect 
that the step-wise approach reduces the computational complexity (see \cite{Denef:2006ad, Halverson:2018cio} for an in-depth discussion of the arising challenges). 
Furthermore, it would be exciting to combine our approach with recent efforts to use machine learning algorithms in studying the 
string landscape \cite{Abel:2014xta, Ruehle:2017mzq, Halverson:2019tkf, Betzler:2019kon, Cole:2019enn, AbdusSalam:2020ywo,CaboBizet:2020cse, Bena:2021wyr, Krippendorf:2021uxu}.

In this work we have also argued that our strategy can be directly extended to F-theory flux compactifications on Calabi-Yau fourfolds. We have 
given the relevant information needed to generally determine the sl(2)$^n$-representation and boundary Hodge decomposition which 
includes the relations in appendix \ref{fourfold_rel}. 
To prepare for giving an explicit example, we then specialized to the large complex-structure regime where the defining information 
of the scalar potential can be given in terms of the topological data of the mirror fourfold. The example that we studied in detail 
was the Calabi-Yau fourfold geometry considered in  \cite{Marchesano:2021gyv} and we focused on the realization of the so-called linear moduli stabilization scenario. 
In order to analyze this geometry from the perspective of asymptotic Hodge theory, we computed the nilpotent orbit and then determined the 
sl(2)-approximation.
We then required the tadpole contribution of the fluxes to remain parametrically finite in the strict asymptotic regime, leading to constraints on the flux quanta matching with \cite{Marchesano:2021gyv}. Subsequently we investigated the stabilization of moduli in the various degrees of approximation at our disposal. In the sl(2)-approximation only one combination of saxions was stabilized (while it already fixes all axions), and by systematically including subleading corrections we could check how the remaining flat directions were lifted. In particular, we reaffirmed the importance of 
the coefficient $K_L^{(3)}$ that is included when going form the sl(2)-approximation to the nilpotent orbit. This correction reduces to the Euler characteristic term in the type IIB case. Restricting 
to cases in which it vanishes we found sets of flux vacua that are real lines stretching to the boundary.
 
Based on this analysis of the linear scenario we also made some additional observations related to recent swampland conjectures and finiteness results. 
Firstly, we noted that describing all vacuum loci in a systematic fashion requires one to go beyond the usual algebro-geometric tools, and instead prompts one to use techniques furnished by tame topology and o-minimality \cite{Bakker:2021uqw,Grimm:2021vpn}. We argued that, as it has to be the case, the linear scenario satisfies the finiteness theorem of \cite{Bakker:2021uqw}. 
Secondly, we pointed out that flux vacua being real lines stretching to the boundary provide us with interesting examples that decouple axions from their counterparts, allowing for infinite distance limits that could serve as non-trivial testing grounds for the axionic string conjecture of \cite{Lanza:2020qmt, Lanza:2021qsu}, the convex hull distance 
conjecture \cite{Calderon-Infante:2020dhm}, and the claims on supersymmetric protection \cite{Palti:2020qlc}. Thirdly, we investigated the validity of the tadpole conjecture \cite{Bena:2020xrh} for the linear scenario. By using statistical arguments following \cite{Plauschinn:2021hkp} we were able to confirm that, under certain genericity assumptions, these models are compatible with the tadpole conjecture. These results suggest that the linear scenario provides no inherent structure to generically 
give counter-examples to the tadpole conjecture --- if one aims to find such a counter-example, one would have to perform a 
thorough search through the available Calabi-Yau databases. It remains an open question whether an explicit 
counter-example exists. 



Let us close by commenting on some further directions that exploit the general nature of our approach. 
To begin with, we can delve deeper into step (1) of our approximation scheme, the sl(2)-approximation. By using the classification of boundaries one can turn moduli stabilization into an abstract problem: the extremization conditions are a simple set of polynomial equations, and the allowed exponents are fixed by the possible boundary types. We can then determine at which boundaries the 
sl(2)-approximation stabilizes all moduli. 
For two-moduli fourfolds this has already been worked out in \cite{Grimm:2019ixq}, but a more general investigation is still missing. 
For step (2) of our scheme, the nilpotent orbit approximation, there is also an abstract approach left unexplored. It has recently been shown that based on \cite{CKS} 
the corrections completing the sl(2)-approximation into the nilpotent orbit approximation can also be incorporated systematically 
by using the holographic perspective put forward in \cite{Grimm:2020cda, Grimm:2021ikg}. It would be interesting to study moduli stabilization using the same strategy. 
Finally, we note that our in our search for flux vacua with approximation steps (1) and (2) we have only included polynomial corrections and essential exponential corrections. 
Finding exact vacua including the whole series of exponential corrections remains a challenging open task. Luckily, in the asymptotic regime, we can judge how 
close we are to the full answer due to the existence of the outlined approximation scheme.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subappendices}

\section{Sl(2)-approximation for linear scenario example}\label{app:linearscenario}
In this section we summarize the relevant building blocks for the sl(2)-approximated Hodge star \eqref{boundarystar}. This consists of the weight and lowering operators $H_i, N^-_i$ of the $\mathfrak{sl}(2)$-triples, and the boundary Hodge star $C_\infty$.
The weight operators are given by
\begingroup
\def\myFigureScale{0.62}
\allowdisplaybreaks
\eq{
\label{linear_operators_weights}
\scalebox{\myFigureScale}{$N^0_0$} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & -2 & -3 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & -2 & -4 & -6 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & -3 & -6 & -6 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & -1 & -2 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
\end{array}
\right) , $}
\\
\scalebox{\myFigureScale}{$N^0_L$} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & -1 & -2 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 2 & -1 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 1 & 0 & -1 & 0 & 2 & 3 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -2 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 2 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & -1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
\end{array}
\right), $}\\
\scalebox{\myFigureScale}{$N^0_1$} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 2 & 1 & 2 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & -1 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -2 & 1 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 1 & -1 & 2 & 2 & 3 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 2 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -2 & 2 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -2 & 1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 1 & -1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
\end{array}
\right),$}\\
\scalebox{\myFigureScale}{$N^0_2$} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 2 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 2 & 4 & 2 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 1 & 1 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & -1 & 2 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
\end{array}
\right).$}
}
The lowering operators are given by
\eq{
\scalebox{\myFigureScale}{$N_0^-$} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \frac{1}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & -1 & -\frac{3}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -4 & -1 & -2 & -3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -\frac{9}{2} & -\frac{3}{2} & -3 & -3 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -\frac{1}{2} & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -\frac{1}{2} & -1 & 2 & 4 & \frac{9}{2} & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 1 & \frac{3}{2} & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 1 & 2 & 3 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & \frac{3}{2} & 3 & 3 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & \frac{1}{2} & 1 & 0 \\
\end{array}
\right) ,$}\\
\scalebox{\myFigureScale}{$N_L^- $} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -3 & 0 & -1 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
\end{array}
\right),$} \\
\scalebox{\myFigureScale}{$N_1^- $} &\scalebox{\myFigureScale}{$= \left(
\begin{array}{cccccccccccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -3 & -1 & -1 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 1 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -1 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & -1 & 0 & 0 \\
\end{array}
\right),$} \\
\scalebox{\myFigureScale}{$N_2^- $} &\scalebox{\myFigureScale}{$=\left(
\begin{array}{cccccccccccccccc}
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 \frac{1}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & -1 & -\frac{1}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -4 & -1 & -2 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -\frac{5}{2} & -\frac{1}{2} & -1 & -\frac{1}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & \frac{1}{2} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{2} & -1 & 0 & 0 & \frac{1}{2} & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -\frac{1}{2} & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & -2 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -\frac{1}{2} & -1 & -\frac{1}{2} & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & \frac{1}{2} & -1 & 0 \\
\end{array}
\right).$}
}
Finally, the Hodge star operator of the boundary Hodge structure is given by
\eq{
\scalebox{\myFigureScale}{$
C_\infty = \left(
\begin{array}{cccccccccccccccc}
 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 1 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & -2 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 2 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 2 & 4 & 2 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & -1 & 1 & 1 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & -1 & 2 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 1 & 0 \\
 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
\end{array}
\right).$}
}
\endgroup

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\end{subappendices}

==> appendices.tex <==
\chapter{Operator relations for Calabi-Yau fourfolds}\label{fourfold_rel}
In the construction of the sl(2)-approximation two operators $\eta$ and $\zeta$ appear, which can be expressed componentwise in terms of $\delta$ with respect to the decomposition \eqref{delta_decomp}. In this appendix we summarize these relations for Calabi-Yau fourfolds. For the purposes of this work we only need $\zeta$, but the expressions for $\eta$ are included for completeness.

Recall that the central identity relating the three operators was given by \eqref{delta-zeta-eta-review}. In the mathematics literature \cite{Kato} this was solved for the components of $\zeta$ for threefolds.\footnote{Furthermore, general expressions for the components $\zeta_{-p,-q}$ and $\eta_{-p,-q}$ in terms of $\delta_{-p,-q}$ were derived, modulo commutators of $\delta_{-r,-s}$ ($r\leq p$ and $s\leq q$) left undetermined.} These results were extended in \cite{Grimm:2021ikg}, where the components of $\eta$ were given in the threefold case. Following the strategy of these works \cite{Kato, Grimm:2021ikg}, we proceed and derive the componentwise expressions for $\eta$ and $\zeta$ for fourfolds. We refer to these articles for a more detailed explanation on how to work out these operator relations. We can express $\zeta$ componentwise in terms of $\delta$ as
\begin{footnotesize}
\begin{align}\label{fourfold_zeta}
 \zeta_{-1,-1}&= \zeta_{-2,-2}= 0\, , \quad \zeta_{-1,-2}= -\frac{i}{2} \delta_{-1,-2}\, , \quad \zeta_{-1,-3} = -\frac{3i}{4} \delta_{-1,-3}\, ,  \quad \zeta_{-1,-4} = -\frac{7i}{8} \delta_{-1,-4}\, ,\nn  \\
\zeta_{-2,-3} &=-\frac{3i}{8} \delta_{-2,-3}+ \frac{1}{8} [\delta_{-1,-2}, \delta_{-1,-1} ]\, , \qquad \zeta_{-2,-4} = -\frac{5i}{8} \delta_{-2,-4} + \frac{1}{4} [ \delta_{-1,-3}, \delta_{-1,-1} ]\, , \nn
\\
 \zeta_{-3,-3} &= \frac{1}{8}[\delta_{-2,-2}, \delta_{-1,-1}]\, ,  \\
\zeta_{-3,-4}  &= -\frac{5i}{16} \delta_{-3,-4} +\frac{3}{16} [\delta_{-2,-3} , \delta_{-1,-1} ] +\frac{3}{16} [\delta_{-1,-3}, \delta_{-2,-1} ] +\frac{i}{48} [\delta_{-1,-1}, [\delta_{-1,-1}, \delta_{-1,-2}]]\, ,  \nn \\
\zeta_{-4,-4} &= \frac{3}{16} [ \delta_{-3,-3}, \delta_{-1,-1} ] +\frac{3}{32} [\delta_{-3,-2} , \delta_{-1,-2}]+\frac{3}{32} [\delta_{-2,-3} , \delta_{-2,-1}]+\frac{i}{32} [\delta_{-1,-1}, [\delta_{-2,-1}, \delta_{-1,-2} ]] \, , \nn
\end{align}
\end{footnotesize}
while $\eta$ is expressed componentwise as
\begin{footnotesize}
\begin{align}\label{fourfold_eta}
\eta_{-1,-1} &= - \delta_{-1,-1}\, , \qquad \eta_{-1,-2} = - \delta_{-1,-2}\, , \qquad \eta_{-1,-3} = - \frac{3}{4}\delta_{-1,-3}\, , \qquad \eta_{-1,-4} = - \frac{1}{2}\delta_{-1,-4}\, , \nn \\
 \eta_{-2,-2} &= - \frac{3}{2} \delta_{-2,-2}\, , \hspace{125.5pt} \eta_{-2,-3} = -\frac{3}{2} \delta_{-2,-3}+\frac{i}{2} [\delta_{-1,-1}, \delta_{-1,-2}]\, , \nn  \\
 \eta_{-2,-4} &= -\frac{5}{4} \delta_{-2,-4}+\frac{5i}{8}[\delta_{-1,-1}, \delta_{-1,-3}]\, , \hspace{30.5pt} \eta_{-3,-3} =  -\frac{15}{8}\delta_{-3,-3}+\frac{5i}{4}[ \delta_{-2,-1}, \delta_{-1,-2}] \, , \nn \\
 \eta_{-3,-4} &= -\frac{15}{8} \delta_{-3,-4}+\frac{3i}{8}[ \delta_{-1,-1},  \delta_{-2,-3}]  \\
 &\quad+\frac{3i}{2}[ \delta_{-2,-1},  \delta_{-1,-3}]+\frac{3i}{4}[ \delta_{-2,-2},  \delta_{-1,-2}] +\frac{1}{8} [  \delta_{-1,-1}, [ \delta_{-1,-1},  \delta_{-1,-2}]]\, , \nn  \\
   \eta_{-4,-4} &= -\frac{35}{16} \delta_{-4,-4} +\frac{63i}{32} [\delta_{-3,-1}, \delta_{-1,-3}]+\frac{21i}{16} [\delta_{-3,-2}, \delta_{-1,-2}]+\frac{21i}{16} [\delta_{-2,-1}, \delta_{-2,-3}] \nn \\
   & \quad +\frac{7}{48}[\delta_{-1,-1},  [\delta_{-1,-1}, \delta_{-2,-2}]]+\frac{7}{24}[\delta_{-2,-1},  [\delta_{-1,-1}, \delta_{-1,-2}]]+\frac{7}{24}[\delta_{-1,-2},  [\delta_{-1,-1}, \delta_{-2,-1}]]\, . \nn
\end{align}
\end{footnotesize}

==> smallW0.tex <==



%Flux compactifications of Type IIB string theory provide some of the best understood scenarios that can yield minimally supersymmetric or non-supersymmetric four-dimensional effective actions with partially or fullystabilized moduli \cite{Grana:2005jc,Douglas:2006es}. These scenarios use the fact that background R-R and NS-NS three-form fluxes introduce a non-trivial superpotential that depends on the complex structure deformations of the internal compactification space and the axio-dilaton. Remarkably, the backreaction of these fluxes on the geometry yields at leading order only a warp factor and the requirement to consider a conformal Calabi-Yau background combined with an orientifold projection. The effective theories can thus be studied by appropriately extending the techniques used to describe the geometry of Calabi-Yau threefolds and their moduli spaces.This has lead to the suggestion of concrete moduli stabilization scenarios in \cite{Giddings:2001yu,Kachru:2003aw,Balasubramanian:2005zx}. The search for explicit realizations of these scenarios still tests our understanding of string compactifications and pushes the boundaries of what is possible or impossible within string theory. 

In this work we will investigate the stabilization of complex structure moduli after introducing background fluxes. 
Following the well-known dimensional reduction on a Calabi-Yau orientifold \cite{Grana:2005jc,Douglas:2006es,Giddings:2001yu,Grimm:2004uq}, we recall that the effective theory is an $\cN=1$ supergravity theory. The for us relevant part of the $\cN=1$ superpotential and K\"ahler potential can be evaluated by determining how the (up to rescaling) unique $(3,0)$-form $\Omega$ on the Calabi-Yau threefold $Y_3$ varies with a change of the complex structure. This dependence can be captured by so-called period integrals, or periods for short, which are obtained by integrating $\Omega$ over a basis of three-cycles of $Y_3$.
There are a number of techniques available to derive these period integrals. 
While most of them require the explicit construction of the Calabi-Yau manifold, it was recently shown in \cite{Bastian:2021eom}
that general models for the asymptotic periods can be constructed by asymptotic Hodge theory. In a nutshell, this 
mathematical formalism uses the existence of monodromy symmetry, the requirement of positivity and orthogonality, and a notion of completeness. It then allows for the construction of the compatible periods with these properties in an algorithmic way 
without resorting to any specific geometric examples. With these powerful techniques at hand we aim to 
understand how certain properties of the effective theory, such as the vacuum expectation value 
of the superpotential and mass hierarchies of the stabilized moduli can be engineered algorithmically. 

One of the most prominent moduli stabilization scenarios, the KKLT scenario \cite{Kachru:2003aw}, requires to find vacua in 
complex structure moduli space, such that the vacuum superpotential is taking a very small, non-zero value.  
It was recently suggested in \cite{Demirtas:2019sip} and further explored in \cite{Demirtas:2020ffz,Blumenhagen:2020ire,Honma:2021klo,Demirtas:2021nlu, Demirtas:2021ote,Broeckel:2021uty} that, in fact, exponentially small vacuum 
superpotentials can be found near certain boundaries in moduli space.\footnote{See \cite{Denef:2004ze, Eguchi:2005eh} for statistical arguments about the abundance of vacua in these regions.} It was argued that the construction proceeds 
by introducing fluxes that preserve a continuous version of the monodromy symmetry at some leading order with a vanishing 
superpotential, while then including instanton corrections generates an exponentially small superpotential. We will 
explain how this construction is understood in asymptotic Hodge theory and how it can be generalized to other boundaries that 
have not been consider in the literature before. This will be done both in a hands-on way by considering explicit examples as well as by explaining how the abstract mathematical methods are useful. 
We will then see that our powerful techniques also allow us to control the moduli masses and 
identify alternative scenarios to the ones of \cite{Demirtas:2019sip,Demirtas:2020ffz}. In our constructions the scaling 
of the masses is polynomial, rather than exponential, in the vacuum expectation values of the moduli. 
In general, the Hodge theory methods enable us to highlight conceptual 
features of these moduli stabilization scenarios and show how to implement them as a building block on general moduli spaces. 
In the mathematical literature, the vacua with 
exponentially small superpotential are a special case of the so-called
extended locus of Hodge classes \cite{schnell2014extended}. 

To highlight some key aspects of our construction let us first point out that asymptotic Hodge theory gives a 
general way of modeling the asymptotic periods of $\Omega$. Firstly, there is the famous result \cite{Schmid}
that ensures that the leading polynomial part of the periods is captured by the monodromy symmetry and some 
data associated to the asymptotic regime. For example, in the large complex structure regime of a 
one-dimensional moduli space the asymptotic periods can be written as $\Pi_{\rm pol} = e^{tN} a_0 
$, where $t$ is the complex structure modulus with $t = i\infty$ being the large complex structure point, $N$ is the logarithm 
of the monodromy matrix and nilpotent $N^4=0$, and $a_0$ is a vector associated to the limit. This form naturally generalizes to 
all limits in complex structure moduli space in one or more directions. Secondly, it was shown in \cite{Bastian:2021eom} that away from the large complex structure regime 
exponential corrections to $\Pi_{\rm pol} $ are needed both for mathematical consistency as well as for the physical effective theory to be well-defined.  
We will thus split the asymptotic periods as $\Pi_{\rm pol} + \Pi_{\rm ess}$ and refer to the corrections $\Pi_{\rm ess}$ as \textit{essential instantons}. This name can be motivated by 
mirror symmetry, where at the large complex structure point exponential corrections actually map to instanton corrections in the mirror theory.  
The necessity of these corrections can be seen, for example, when the metric derived solely from $\Pi_{\rm pol}$  degenerates. Remarkably, the 
asymptotic Hodge theory techniques introduced  in \cite{Schmid,CKS,CKAsterisque} can then be used to determine the general form of the needed  exponentially suppressed corrections $\Pi_{\rm ess}$
to exactly avoid such inconsistencies. 


With these insights about the structure of the periods we  search for flux vacua that admit exponentially small vacuum superpotentials. 
Using the classification of asymptotic regimes \cite{Kerr2017,Grimm:2018cpv,Grimm:2019bey} we are able to identify a specific class of regions that 
generally admits essential instanton corrections that can set the scale of the vacuum superpotential. 
We find that a large class of such regions arise near boundaries containing Seiberg-Witten points. These special 
loci occur in the moduli space of Calabi-Yau geometries that are used to embed Seiberg-Witten theory into type IIB string theory \cite{Kachru:1995fv,Eguchi:2007iw}. 
Among the set of essential instantons in the flux superpotential we then identify a subset that enters the 
scalar potential already at polynomial order. These are 
precisely the instanton corrections that are required to ensure a non-degenerate moduli metric and induce  the polynomial behavior of the moduli masses in the vacuum. We refer to these corrections as \textit{metric-essential instantons} in this paper. 
Furthermore, we then find that in these vacua the canonically 
normalized masses of the axio-dilaton and complex structure moduli can be parametrically heavier 
compared to the mass of the K\"ahler moduli.

 In order to illustrate our method, we then specialize our analysis to one and two moduli settings. General models for the asymptotic periods of these low-dimensional settings have recently been constructed in \cite{Bastian:2021eom} and we will use them here to perform explicit computations. It turns out that these concrete realizations lead to additional intriguing observations about the hierarchies among moduli masses and the minimal scale of the vacuum superpotential. While we are not providing any general proofs on these findings, they are suggestive of a deeper structure and provide additional motivation for an explicit study of higher dimensional examples. Finally, we should mention that the period models used in this work are given in a real rather than a rational symplectic basis. Our vacua do not require any fine-tuning of the flux quanta in contrast to e.g.~a racetrack potential, so we do not expect any technical issues to arise here. Nevertheless it would be interesting to work out the quantization of the fluxes in the future.

The paper is organized as follows. In section \ref{sec:IIBflux} we review some basic aspects of Type IIB flux compactifications, and outline our strategy for constructing vacua with exponentially small superpotentials. Particularly, we review how essential instantons can play a crucial role in e.g.~the K\"ahler metric, and explain how to carefully deal with these corrections in the context of moduli stabilization. In section \ref{sec:examples}, to illustrate this story further, we then consider two simple examples, where we show how to stabilize the moduli explicitly such that we engineer an exponentially small vacuum superpotential. In section \ref{sec:conclusions} we present our conclusions and give promising directions for future research.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Type IIB flux compactifications and small superpotentials}\label{sec:IIBflux}













\subsection{Engineering vacua with small $W_0$}
\label{ssec:strategy}
We now lay out our strategy for engineering vacua with a small flux superpotential. This construction relies on first searching for solutions to the F-term equations coming from the polynomial periods $\Pi_{\rm pol}$ and supplementing them accordingly with constraints involving essential instantons in order to stabilize all moduli. As a result we will have $W_{\rm pol}=0$ and consequently an exponentially small vacuum superpotential $W_0$. This procedure is then explicitly applied to the one- and two-moduli type $\rm II$ models in sections \ref{ssec:II0} and \ref{ssec:II1} respectively.

Let us begin by writing down the relevant extremization conditions at polynomial level for our flux vacua. As we want to engineer vacua with an exponentially small superpotential, we require the polynomial part in the expansion of the superpotential \eqref{eq:Wexpansion} to vanish
\begin{equation}
W_{\rm pol} \big|_* = 0\, ,
\end{equation}
where we used a star to denote the evaluation of moduli at their vevs. At the polynomial level of the superpotential the vanishing F-term constraints \eqref{eq:Fterms} can then be written as
\begin{equation}\label{eq:polextr}
\begin{aligned}
  \langle F_3 - \tau_* H_3 , \,  \,  e^{t^i_* N_i} N_a a_0 \rangle = 0\, , \qquad \langle H_3 , \, e^{t^i_* N_i} a_0 \rangle = 0\, ,  \qquad \langle F_3 , \, e^{t^i_* N_i} a_0 \rangle = 0\, .\\
\end{aligned}
\end{equation}
The first set of equations follows from $\partial_a W_{\rm pol} \big|_* = 0$, while the latter two follow from $\partial_\tau W_{\rm pol}  \big|_*= 0$. Note that we replaced the covariant derivative by a partial derivative for all constraints since $W_{\rm pol}\big|_*  = 0$ for the flux vacua we are interested in.

It is important to stress that these polynomial level conditions \eqref{eq:polextr} do not suffice to obtain the vacua of 
the scalar potential. The vectors $N_a a_0$ can be parallel or even vanishing resulting in a insufficient set of F-term conditions at the polynomial level. Another way to observe this is by looking at the scalar potential $V_{\rm pol}$ obtained from the complete $V$ defined in \eqref{eq:potential} 
by dropping all exponentially suppressed corrections in the final expression. We now look for a combination $\phi$ of moduli that is not constrained by 
the condition  \eqref{eq:polextr}. If such an unfixed direction $\phi$ exists, two possibilities can occur:
\begin{itemize}
\item[(1)] The direction $\phi$ is a flat direction of the polynomial scalar potential $V_{\rm pol}$. This implies that $\phi$ is massless at polynomial order, but might obtain an exponentially small mass upon including either essential or non-essential instanton corrections. 
\item[(2)]  The direction $\phi$  is \textit{not} a flat direction of the polynomial scalar potential $V_{\rm pol}$, but rather has a mass term already at polynomial order. This implies that their mass term must arise from \textit{metric-essential instantons} correcting the periods. 
\end{itemize}
Let us comment on these two cases in turn. First, note that for case (1) the field $t_*$ not appearing in $V_{\rm pol}$ might still be stabilized after including instanton corrections. If non-essential instantons are used in order to ensure the stabilization one needs 
to check if such corrections are actually present for a given Calabi-Yau geometry and implement an appropriate stabilization scheme, such as a racetrack potential. To make this concrete in explicit examples was one of the successes of \cite{Demirtas:2019sip,Blumenhagen:2020ire,Demirtas:2020ffz}. In particular, it was shown that this can be done at large complex structure point in \cite{Demirtas:2019sip}. While there are no essential instantons in this asymptotic limit, it is well-known that generically instanton corrections arise and contribute to the superpotential. Second, we note that realization of case (2) is primarily dependent only on the type of asymptotic regime, since we have a systematic classification in which asymptotic regime certain essential instanton corrections have to be present. One has thus a stabilization mechanism that is independent of the actual Calabi-Yau geometry that realizes this limit. In the following we will focus on case (2) and explain in detail how such situations can be engineered. 

To gain a better understanding of what happens in case (2), let us note that such vacua exactly arise if 
the polynomial part of the K\"ahler potential $\cK_{\rm pol}$ yields a degenerate K\"ahler metric, i.e.~when the full K\"ahler metric has exponential eigenvalues. To see this we 
recall from the discussion below \eqref{eq:Wexpansion} that such a K\"ahler metric allows exponentially suppressed contributions in the F-terms to enter the scalar potential \eqref{eq:potential} at polynomial order. Hence, the stabilization of the moduli at polynomial order 
requires a more careful treatment of the complete F-terms supplementing \eqref{eq:polextr} by additional constraints coming from metric-essential instantons. 

Let us outline an approach to read off these additional constraints by a more careful treatment of the F-terms. 
The exponentially suppressed contributions in the F-terms appear in the polynomial scalar potential through exponential eigenvalues of the K\"ahler metric, so it is convenient to expand $D_I W$ in an eigenbasis for the K\"ahler metric. The eigenvectors relevant for the supplementary constraints then have a vanishing eigenvalue under the polynomial part of the K\"ahler metric 
\begin{equation}
(\partial_i \bar{\partial}_{\bar{\jmath}}\log \cK_{\rm pol}) V^j = 0\, ,
\end{equation}
For boundaries with a linear $\cK_{\rm pol}$ such as in section \ref{ssec:II1} these eigenvectors $V^i$ will always be independent of the saxions, but for more general boundaries this need not be the case. Letting $a_{r_1 \cdots r_n}$ denote the essential instanton term corresponding to a given eigenvector $V^i$, then the relevant F-term constraint can be written as
\begin{equation}\label{eq:expextr}
V^i D_i W =V^i \partial_i W_{\rm inst} =  e^{2\pi i r_i t^i} \langle F_3 - \tau_* H_3, \, V^i (2\pi i  r_i + N_i) e^{t^i_* N_i} a_{r_1 \cdots r_n} \rangle = 0 \, ,
\end{equation}
where we used that $V^i \partial_i W_{\rm pol}=0$, and replaced the covariant derivative by a partial derivative because $V^i K^{\rm cs}_i \, W_{\rm inst}$ is subleading in the instanton expansion. Furthermore, note that we dropped correction terms subleading compared to the essential instanton $a_{r_1 \cdots r_n}$. The complete set of extremization conditions to stabilize the moduli at polynomial order of the scalar potential is then given by \eqref{eq:polextr} and as many equations of the form \eqref{eq:expextr} as there are metric-essential instantons. Since the exponential factor in \eqref{eq:expextr} is simply an overall factor, this yields a system of polynomial equations in the moduli.\footnote{This polynomial structure of the extremization conditions is natural from the perspective of the self-duality condition \eqref{eq:selfduality}. The dependence on the complex structure moduli then enters through the Hodge star operator, whose polynomial part is already non-degenerate as discussed below \eqref{eq:Wexpansion}. }



An interesting feature of the vacua constructed according to the above scheme is a natural hierarchy of mass scales. All moduli are stabilized by the polynomial part of the scalar potential, so the eigenvalues of the hessian $\partial_I \partial_J V$ will be polynomial as well. Recall that the inverse K\"ahler metric either has polynomial or exponentially large eigenvalues, and that the canonically normalized masses are then computed as the eigenvalues of $K^{IC} \partial_C \partial_J V$. This means that the moduli masses take polynomial or exponentially large values in the vevs of the saxions. Either way, this separates the mass scale of the complex structure moduli and the axio-dilaton from the exponentially small scale of $|W_0|^2$. This hierarchy makes our flux vacua particularly attractive from the perspective of the KKLT scenario \cite{Kachru:2003aw}, since it allows one to consistently integrate out the complex structure and axio-dilaton sector before dealing with the K\"ahler moduli. This point separates our construction from other findings \cite{Demirtas:2019sip,Blumenhagen:2020ire,Demirtas:2020ffz}, where the mass of the lightest complex structure modulus was of the same scale then $|W_0|^2$, requiring a more refined analysis. 

We end this general discussion by commenting on the application of our procedure near the different types of boundary points. Given a type $\rm I$ point our method does not work. Roughly speaking, this is due to the fact that there is too little information contained in the polynomial piece of the period vector and as a consequence there is not enough freedom in the fluxes to stabilize all moduli at the polynomial level of the scalar potential as a result. We elaborate on this point in  appendix  \ref{finite_distance_appendix}. Near type $\rm II$ points, we have a polynomial K\"ahler potential that is at most linear in the complex structure moduli, which makes it the simplest and most natural candidate for our procedure. In section \ref{ssec:II0} and \ref{ssec:II1}, we explicitly apply our method to the one and two moduli cases respectively. A type $\rm III$ point does not occur in complex structure moduli spaces of dimension less than three. As the models developed in \cite{Bastian:2021eom} only had a maximum of two moduli, we did not have an explicit realization of this scenario at our disposal. There is, however, no obvious reason for which the construction should not go through in that case. For a type $\rm IV$ that is not at LCS, the simplest scenario occurs for two moduli. In that case there is a technical obstruction to the success of our method, but this problem should be solvable given more than two moduli. These last two types deserve more concrete investigations in the future and we make some further comments about them in the conclusions.





\section{Explicit models}\label{sec:examples}
In this section we illustrate our method for finding flux vacua with exponentially small superpotentials by studying one- and two-moduli boundaries in complex structure moduli space. Our search uses asymptotic models for the periods near these boundaries constructed in \cite{Bastian:2021eom}, and we refer the reader to this work for more details about their construction and conventions. We emphasize that, since all possible one- and two-moduli boundaries have been classified \cite{Kerr2017,Grimm:2018cpv,Bastian:2021eom}, this construction yielded an exhaustive set of asymptotic periods. For completeness let us recall some aspects of this classification. For one modulus, we can have three main types I, II, IV at point-like boundaries. In the two-dimensional case the picture already 
becomes richer, since two one-dimensional boundaries can intersect in a point. At this intersection point again only the three types I, II, IV can occur. If this 
type is IV, then there are two classes of intersections: (1) the familiar large complex structure cases, (2) the so-called coni-LCS cases. 
Near both of these intersections exponentially small superpotentials have already been constructed by considering specific geometric examples in \cite{Demirtas:2019sip,Demirtas:2020ffz,Blumenhagen:2020ire}. We refer to these works for a detailed treatment. 
This leaves us with the intersections where one encounters the types I or II at the intersection point. The Type I boundaries are at finite distance and we will 
discuss in appendix \ref{finite_distance_appendix} that one cannot stabilize all moduli at the level of the polynomial scalar potential in these situations. This implies that we would need to include further 
non-essential instanton corrections to stabilize a remaining polynomially flat direction.  This leaves us with the class of $\mathrm{II}$ boundaries, and we investigate how to engineer exponentially small vacuum superpotentials near these boundaries in the following. 





\subsection{One-modulus  asymptotic region near a type $\mathrm{II}$ point}\label{ssec:II0}
We start with the simplest case, namely the one-modulus asymptotic regions that are near type $\mathrm{II}$ boundaries. 
These have already been systematically studied in the math literature \cite{Tyurin:2003}, and such boundaries correspond to so-called Tyurin degenerations. The period vectors near these boundaries have been computed for an explicit example in the physics literature in \cite{Joshi:2019nzi}, and general models for these periods including essential instantons have been constructed in \cite{Bastian:2021eom}. Using the results from the latter, we find that the K\"ahler potential \eqref{eq:kahlerexpansion} takes the form
\begin{equation}\label{eq:kpII0}
\cK_{\rm pol}=4  y \, , \qquad \cK_{\rm inst} =  \frac{4  a^2(1+\pi y)}{\pi} e^{-4 \pi y} \, , 
\end{equation}
where $a \in \mathbb{R}_{\neq 0}$ is some model-dependent coefficient that controls the essential instanton term and we have dropped all the non-essential instanton corrections. The polynomial and exponential parts of the flux superpotential take the respective forms
\begin{equation}\label{eq:WII0}
\begin{aligned}
W_{\rm pol}&=-g_3-ig_4+(g_1+ig_2)t \, ,\\
W_{\rm inst}&=a \, e^{2\pi i t}(t-\frac{1}{\pi i})(g_1-ig_2)-a \, e^{2\pi i t}(g_3-ig_4)\, ,
\end{aligned} \,
\end{equation}
where the $g_i = f_i - \tau h_i$ are the components of the three-form fluxes with $\tau = c+is$ being the axio-dilaton. We now proceed to stabilizing the moduli at the polynomial level. The vanishing F-term conditions for the polynomial part of the flux superpotential can conveniently be written as
\begin{equation}\label{eq:DWII0}
\begin{aligned}
y D_t W_{\rm pol} - s D_\tau W_{\rm pol} &= (f_1+i f_2) y - (h_3+i h_4) s=0\, , \\
y D_t W_{\rm pol} + s D_\tau W_{\rm pol} &= -i(f_3+i f_4) -i  (h_1+i h_2) sy =0\, , 
\end{aligned}
\end{equation}
where we dropped exponentially suppressed terms and set the axions to zero, i.e.~$c=x=0$. We chose not to impose $W_{\rm pol}=0$ at first, leaving us with the full covariant derivatives at polynomial level in the above extremization conditions. The solution to these constraints is given by
\begin{equation}\label{eq:vevsII0}
s = \sqrt{-\frac{f_1 f_3}{h_1 h_3}}\, , \qquad y = \sqrt{-\frac{ f_3 h_3}{f_1 h_1}}\, , \qquad f_2 h_3 = f_1 h_4\, , \qquad f_4 h_1 = f_3 h_2\, , 
\end{equation}
where we require $f_1/h_3 >0$ and $f_3/h_1<0$ in order to get positive values for the saxions. Plugging this solution back into the superpotential \eqref{eq:WII0} we find that $W_{\rm pol} = 0$ holds when
\begin{equation}
h_2 =- f_1 \sqrt{-\frac{h_1 h_3}{f_1 f_3}}\, , \qquad h_4 = - f_3 \sqrt{-\frac{h_1 h_3}{f_1 f_3}}\, . \label{eq:II0Const2}
\end{equation}
Implementing the constraints \eqref{eq:vevsII0} and \eqref{eq:II0Const2}, we obtain flux vacua that have $W_{\rm pol}=0$. Thus, the scale of the superpotential is set by 
\begin{align}
|W|=|W_{\rm inst}| \sim a \, e^{- 2 \pi y} = a  \exp\Big(-2\pi \sqrt{-\frac{ f_3 h_3}{f_1 h_1}}\, \Big)\, .
\end{align}
We want to emphasize that the exponentially small scale of the superpotential is set by an essential instanton term that is required by consistency of the theory, i.e.~the coefficient $a$ cannot vanish for any geometric example. Furthermore, we can now relate the saxion masses and their vevs to the tadpole. The latter takes the form
\begin{equation}
Q_{\rm D3}=f_1 h_3 - f_3 h_1 \,.
\end{equation}
Computing the masses from the scalar potential as the eigenvalues of $K^{ac} \partial_c \partial_b V$ we find that they are given by the compact expression
\begin{align}
m_{t}^2=m_{\tau}^2=\frac{1}{\cV^2}(f_1 h_3 - f_3 h_1) =  \frac{Q_{\rm D3}}{\cV^2} \,,
\end{align}
where $m_t^2, m_\tau^2$ denote the canonically normalized moduli masses associated with the complex structure modulus and the axio-dilaton respectively. Let us also stress that this one-modulus case is rather non-generic as there are no metric-essential instantons required, which have to be present in the multi-moduli case as we will see below. Furthermore, the saxion vev $y$ is bounded from above by the tadpole as
\begin{align}
y \leq  2(f_1 h_3-f_3 h_1)= 2 Q_{\rm D3} \,,
\end{align}
which is saturated for $f_3=h_3$ and $f_1=h_1=1$. As the scale of $|W_0|$ is set by $e^{-2 \pi y}$, we cannot make it arbitrarily small by tuning the vev of the saxion $y$, i.e.
\begin{align}\label{eq:W0boundII0}
|W_0| \gtrsim e^{-2 \pi Q_{\rm D3}}\, .
\end{align}
 To be more concrete, we consider a specific set of fluxes that satisfy the above equations. Given $H_3 = (-1,-2,4,-2)$ and $F_3=(8,-4,8,16)$, we find that
\begin{equation}
s = 4\, , \qquad y=2\,, \qquad |W_0 | \sim a \, e^{-4\pi}\, ,\qquad m_t^2 = m_\tau^2 = Q_{\rm D3} =40\, ,
\end{equation}
where we dropped the volume factor $1/\cV^2$ in the masses for convenience.

\subsection{Two-moduli asymptotic region near a type II point}\label{ssec:II1}
Next we consider the more involved class of two-moduli  boundaries that intersect on a type II point. Such asymptotic regions are realized, for example, in the moduli space of the Calabi-Yau threefold in $\mathbb{P}^{1,1,2,2,6}_4[12]$ near a Seiberg-Witten point \cite{Kachru:1995fv, Curio_2001,Eguchi:2007iw,Lee:2019wij}. Using the asymptotic model from \cite{Bastian:2021eom}, we find that the K\"ahler potential \eqref{eq:kahlerexpansion} near these boundaries takes the form
\begin{equation}\label{eq:kpII1}
\begin{aligned}
\cK_{\rm pol} &= 4(y_1+n_2 y_2) \, ,  \\
\cK_{\rm inst} &= -2 a^2 e^{-4\pi y_2} \Big(  n_1 y_1+y_2 + \frac{1-n_1 n_2}{2\pi} \Big) \\
& \ \ \ \, -2 n_2 b^2 e^{-4\pi y_1} \Big( n_2(n_1y_1+y_2) -\frac{1-n_1 n_2}{2\pi} \Big) \\
& \ \ \ \, -4 ab e^{-2\pi y_1-2\pi y_2}\Big(  n_2 ( n_1 y_1+y_2) + \frac{(n_2-1)(1-n_2 n_2)}{4\pi} \Big) \cos(2\pi(x_1-x_2)) \, , \\
\end{aligned}
\end{equation}
where $a,b \in \mathbb{R}_{\neq 0}$ and $n_1,n_2 \in  \mathbb{Q}_{\geq 0}$ are model-dependent parameters that control the essential instanton terms. The polynomial and exponential parts of the flux superpotential take the respective forms
\begin{equation}\label{eq:WII1}
\begin{aligned}
W_{\rm pol} &=  ( g_1+ig_2) (t_1+n_{2}  t_2) +( g_1+i g_2)- (g_4+i g_5)\, ,\\
W_{\rm inst} &=   a \, e^{2\pi i t_2} \Big(ig_3\frac{1-n_1 n_2}{2 \pi } -g_3 n_{1} n_{2}  t_1 - g_3 n_{2} t_2-     g_6 n_{2}\Big) \\
  & \ \ \ +  b \, e^{2\pi i t_1} \Big(ig_3 \frac{n_{1} n_{2}-1}{2\pi}  -g_3 n_{1} t_1 -g_3 t_2 -
   g_6 \Big) +\mathcal{O}(e^{-4\pi y})\,  .
\end{aligned}
\end{equation}
 Let us already point out that the polynomial part of the K\"ahler potential and flux superpotential is very similar to those of the one-modulus $\mathrm{II}_0$ boundaries given in \eqref{eq:kpII0} and \eqref{eq:WII0}, for which we only need to replace $t$ by $t_1+n_2 t_2$ and relabel some of the fluxes. By computing the K\"ahler metric for \eqref{eq:kpII1} one sees that $\cK_{\rm pol}$ yields a degenerate polynomial metric, as elaborated upon below \eqref{eq:example_metric} . This degeneracy is cured by the exponentially suppressed term involving $a^2$ in $\cK_{\rm inst}$, which therefore is a metric-essential instanton. Note that the essential instanton term involving $b$ can also cure this degeneracy unless $n_2=0$. 

Now let us turn to the extremization conditions that have to be solved. The vanishing F-term conditions can conveniently be written as
\begin{equation}\label{eq:DWII1}
\begin{aligned}
(y_1 + n_2 y_2) D_{t_1} W - s D_\tau W &= (y_1+n_2 y_2)(f_1+if_2) -s(h_4+i h_5) = 0\, , \\
(y_1 + n_2 y_2) D_{t_1} W + s D_\tau W &=  -i f_4 +f_5 + s(y_1+n_2 y_2)(-ih_1+h_2)= 0\, , \\
\frac{n_2  D_{t_1} W - D_{t_2} W}{2\pi (a e^{-2\pi y_2}-n_2^2 b e^{-2\pi y_1} ) } &= i f_6 +s h_6 -(n_1 y_1 +y_2) (f_3 - i sh_3) = 0\, .
\end{aligned}
\end{equation}
The first two conditions take a similar form as \eqref{eq:DWII0} found near one-modulus $\mathrm{II}$ boundaries, where the saxion $y$ is now replaced by the linear combination $y_1+n_2 y_2$ and some fluxes are relabeled. Proceeding in the same fashion as the one-modulus setup, these two equations fix the saxions $y_1+n_2 y_2$ and $s$, and furthermore impose two relations on the fluxes that ensure their axionic partners have vanishing vevs
\begin{equation}\label{eq:solve1II1}
y_1+n_2 y_2 =\sqrt{-\frac{ f_4 h_4}{f_1 h_1}} \, , \qquad s =\sqrt{-\frac{f_1 f_4}{h_1 h_4}} \, , \qquad f_2 h_4 = f_1 h_5\, , \qquad f_5 h_1 = f_4 h_2\, ,
\end{equation}
where we require $f_1/h_4 >0$ and $f_4/h_1<0$ in order to get sensible values for the saxions. 

The relevance of the third equation in \eqref{eq:DWII1} is a bit more subtle. While this F-term is exponentially suppressed, it does contribute to the polynomial part of the scalar potential, in line with our discussion at the end of section \ref{ssec:asymptotics}. This can be seen by carefully inspecting the K\"ahler potential \eqref{eq:kpII1}, which yields a K\"ahler metric with an exponentially small eigenvalue for the eigenvector $(n_2, -1)$. This scaling then cancels against the scaling of the F-term when computing the scalar potential through \eqref{eq:potential}, hence contributing at polynomial order. Therefore we must require the third F-term given in \eqref{eq:DWII1} to vanish as well, which is solved by
\begin{equation}\label{eq:solve2II1}
n_1 y_1+y_2 =  \sqrt{-\frac{f_6 h_6}{f_3 h_3}}  \, , \qquad f_3 f_6 h_1 h_4 = f_1 f_4 h_3 h_6\, .
\end{equation}
where we must require $f_3 / h_6 >0$ and $f_6 / h_3 <0$ to have positive saxion vevs compatible with the positivity conditions given below \eqref{eq:solve1II1}.

Together \eqref{eq:solve1II1} and \eqref{eq:solve2II1} specify all vacua (with vanishing axion vevs) of the polynomial scalar potential arising from the flux superpotential \eqref{eq:WII1}. We are interested in constructing vacua with $W_{\rm pol}=0$, which amounts to additionally imposing
\begin{equation}
h_2 = -f_1 \sqrt{-\frac{h_1 h_4}{f_1 f_4}}\, , \qquad h_5 = -f_4 \sqrt{-\frac{h_1 h_4}{f_1 f_4}}\, .
\end{equation}
It is now instructive to compare the scale of the moduli masses and the vacuum superpotential again with the D3-brane tadpole. The tadpole contribution due to the fluxes can be split into two parts as
\begin{equation}
Q_{\rm D3}  = \underbrace{ f_1 h_4-  f_4 h_1}_{Q^{\rm pol}_{\rm D3} }   +\underbrace{\frac{1}{2}( f_3 h_6 -f_6 h_3)}_{Q^{\rm inst}_{\rm D3} }\, , 
\end{equation}
where we separated the fluxes that appear in the superpotential \eqref{eq:WII1} at polynomial order from the fluxes that enter at exponential order. From the positivity conditions on the fluxes given below \eqref{eq:solve1II1} and \eqref{eq:solve2II1} we see that all terms in the contributions $Q^{\rm pol}_{\rm D3}$ and $Q^{\rm inst}_{\rm D3}$ are positive. For the canonically normalized masses of the moduli we then compute the eigenvalues of $K^{ac}\partial_c \partial_b V$ and find that
\begin{equation}
m_\tau^2 = m_{t_1+n_2 t_2}^2 =  \frac{f_1 h_4-  f_4 h_1}{\cV^2} = \frac{Q^{\rm pol}_{\rm D3} }{\cV^2} \leq \frac{Q_{\rm D3}}{\cV^2}  \, ,
\end{equation}
where we dropped the overall volume factor $1/\cV^2$ for convenience. We do not write down the mass associated with the modulus $n_2 t_1 - t_2$ here, but note that it takes an exponentially large value in the fluxes, since this field corresponds to an exponential eigenvalue of the K\"ahler metric. 

For the scale of the vacuum superpotential we need to study the saxion vevs. By using \eqref{eq:solve1II1} and \eqref{eq:solve2II1} we find the following two bounds through the D3-brane tadpole
\begin{equation}
y_1+n_2 y_2 \leq \frac{1}{2}Q^{\rm pol}_{\rm D3}\, ,\qquad n_1 y_1+y_2 \leq Q^{\rm inst}_{\rm D3} 
\end{equation}
which are saturated for $f_1=h_1=1$, $f_4=-h_4$ and $f_3=h_3=1$, $f_6=-h_6$ respectively. The vacuum superpotential is then set by the smallest saxion vev as
\begin{equation}
|W_0| \sim e^{-2\pi \min(y_1,y_2)} \geq e^{-2\pi Q_{\rm D3}}\, .
\end{equation}
Given both this bound on the vacuum superpotential and \eqref{eq:W0boundII0} in the one-modulus setup, it is tempting to speculate that $|W_0|$ can be bounded from below by the D3-brane tadpole near any type II point, also in higher-dimensional moduli spaces. In light of the tadpole conjecture \cite{Bena:2020xrh,Bena:2021wyr} this hints at an interesting tradeoff, where making $|W_0|$ smaller by increasing $h^{2,1}$ runs into problems with achieving full moduli stabilization.


To make the above story more concrete, let us consider the Seiberg-Witten point in the moduli space of the Calabi-Yau threefold in $\mathbb{P}^{1,1,2,2,6}_4[12]$ as an example. Following \cite{Bastian:2021eom}, we find that this boundary corresponds to the monodromy data $n_1=0$, $n_2=1/4$. As flux quanta we pick
\begin{equation}
F_3 = (-4,-8,10,16,-8,-8)\, , \qquad  H_3 = (-2,1,1,-2,-4,5)\, .
\end{equation}
The scalar potential then has a minimum at
\begin{equation}
s = 4\, , \qquad y_1 = 1.5 \, , \qquad y_2 = 2 \, , \qquad |W_0| = 7.3\cdot 10^{-5}\, ,
\end{equation}
where we used that $b=-4 \Gamma(3/4)^4/(\sqrt{3} \pi^2)$, and ignored the coefficient $a$ in the expansion of the superpotential \eqref{eq:WII1} since $e^{-2\pi y_1} \gg e^{-2\pi y_2} $. The canonically normalized moduli masses are then computed to be
\begin{equation}
 m_{n_2 t_1-t_2}^2 = 1.3 \cdot 10^{10} \, , \qquad m_{t_1+n_2 t_2}^2  = m_{\tau}^2 = 40 = Q^{\rm pol}_{\rm D3} \, ,
\end{equation}
where we dropped the volume factor $1/\cV^2$ in the moduli masses for convenience.
Note in particular that there is one exponentially large mass, which corresponds to the eigenvector of the K\"ahler metric with an exponential eigenvalue. Furthermore, all moduli masses are orders of magnitude larger than the exponentially small $|W_0|^2$.







\section{Conclusions}\label{sec:conclusions}
In this paper, we 
described the systematic construction of Type IIB flux vacua with an exponentially small vacuum superpotential 
using recent insights from asymptotic Hodge theory. It is based on the fact that all asymptotic regions in complex structure moduli 
space can be classified \cite{Kerr2017} and that general models for asymptotic period vectors 
can be constructed in each of these regions \cite{Bastian:2021eom}. 
Crucially, this can be done without reference to a specific geometric realization and therefore gives a powerful tool 
to do model-building by directly manipulating the geometry of the moduli space. A crucial aspect of this construction is that the inclusion of  what we called 
essential instantons is important in most asymptotic regimes. These appear as exponential corrections to the polynomial part of the periods and are required  
 by the general statements of asymptotic Hodge theory. Their presence is also of physical significance, since they ensure, for example, that the kinetic terms
 of the complex structure moduli are non-degenerate and positive. In this work we have shown how essential  
 instanton corrections can be the crucial ingredient in obtaining vacua with an exponentially small 
 superpotentials and a hierarchy in the mass matrix of the moduli. 
 
 A first takeaway of our approach to constructing flux vacua is that there is a conceptual difference in whether 
 the exponentially small value of the superpotential is induced by essential or non-essential instantons. Non-essential instantons 
 are not required by consistency, but are well-known to arise in most known explicit geometric examples. They have 
 been central in the flux superpotential constructions of \cite{Demirtas:2019sip,Demirtas:2020ffz,Blumenhagen:2020ire} and lead to mass matrices with exponentially small eigenvalues. 
 In contrast, we showed that the exponential terms induced by essential instantons in the superpotential and K\"ahler potential 
 can combine to contributions to the scalar potential that enter at polynomial level. In fact, a special subset of these instantons, which 
 we termed \textit{metric-essential} since they ensure the non-degeneracy of the moduli metric, necessarily leads to such polynomial 
 corrections in the scalar potential. Remarkably, we were thus able to study moduli stabilization at polynomial level and an 
 exponentially small vacuum superpotential with the control provided by asymptotic Hodge theory. 

To concretely demonstrate how our method works we explicitly applied it to one- and two-dimensional complex structure moduli spaces by singling out a certain set of boundaries and associated asymptotic regions within in the classification of all occurring possibilities of \cite{Kerr2017}. The considered asymptotic regions were close to a Type II point in both 
the one- and two-dimensional moduli spaces, i.e.~we assumed that boundary of the highest co-dimension is of this specific type. 
We showed that in one- and two-dimensional moduli spaces this is a sufficient condition for implementing an exponentially small vacuum superpotential controlled by essential instantons and suspect that this conclusion also generalizes  to higher-dimensional moduli spaces. In the considered low-dimensional examples we have already observed some interesting features of these models. Firstly, we have seen that starting at dimension two the moduli metric always has exponentially small eigenvalues, while the scalar potential can still depend polynomially on the same field. This universal feature of Type II points in moduli space is only absent for the one-dimensional moduli spaces, which are known to be special also from other perspectives \cite{Grimm:2018ohb}. Secondly,  for both one- and two-dimensional moduli spaces, we have found that
one complex structure modulus and the axio-dilaton are stabilized at polynomial order and have a mass of the same order. 
Thirdly, we have shown that in the considered cases there is a simple bound on how small $|W_0|$ can be made. 
It is expected that such a bound exists due to the finiteness of 
flux vacua \cite{Grimm:2020cda, Bakker:2021uqw,Grimm:2021vpn}, but it is interesting that one can show that this bound is set by the exponential of the negative tadpole charge. Concluding this summary, let us note that we expect that most of these observations can also be established for higher-dimensional moduli spaces. 

Let us stress that our approach is of particular use in the realization of certain moduli stabilization scenarios, such as the KKLT scenario. The metric-essential instantons 
provide mass to the complex structure moduli that is naturally larger than the mass scale of the non-perturbatively stabilized K\"ahler structure moduli. 
This avoids the complications arising from dealing with a very light complex structure modulus. However, we note that it is a general feature of the outlined scenario in moduli spaces with $h^{2,1}>1$ that one finds at least one complex structure modulus that gains an exponentially large mass after canonical normalization. This 
is due to the fact that the moduli metric admits an exponentially small eigenvalue set by the metric-essential instantons. It needs to 
be ensured that the mass of this field is still sufficiently below the Kaluza-Klein scale to make our considerations self-consistent. 
One can then aim at implementing an exponentially small vacuum superpotential by including the outlined stabilization 
scheme as a building block in a more extensive setting. For example, one can stabilize a number of the 
complex structure moduli near a Type II boundary and use the essential instantons to control the superpotential. We 
expect that this can be done for explicit geometric Calabi-Yau examples or abstractly by using Hodge theory 
techniques. In either approach the described building block can be part of a general asymptotic moduli stabilization scheme put forward in \cite{Grimm:2019ixq,Grimm:2021ckh}.

There are numerous interesting questions for future research that might be answered using the general understanding of the asymptotic complex structure moduli space. Most immediate is to explore how our construction of flux vacua near Type II points extends to higher-dimensional moduli spaces and more involved boundary configurations. In particular, while we have presented arguments that our construction does not work for finite distance boundaries, there are more possibilities for infinite distance boundaries other than Type II and the large complex structure boundaries. For example, in higher-dimensional moduli spaces one can find novel Type $\mathrm{III}$ boundaries that cannot occur in complex structure moduli spaces of dimension less than three. Furthermore, there are also so-called coni-LCS boundaries, which roughly speaking arise when a finite distance boundary meets an infinite distance boundary. For those our method requires also at least three moduli in order to have enough freedom to stabilize moduli at the polynomial level. This fact ties nicely together with the recent construction of flux vacua near such boundaries in the three moduli setting that have been proposed in \cite{Demirtas:2020ffz,Blumenhagen:2020ire}. The most direct way to make progress on more general configurations is to extend the construction of asymptotic periods in \cite{Bastian:2021eom} and then use them to study flux vacua. Alternatively one can aim to apply the asymptotic Hodge theory techniques directly to the scalar potential as in \cite{Grimm:2019ixq,Grimm:2021ckh}, but this requires one to develop an efficient strategy to gain information about the superpotential. 

Let us close by stressing that the constructions of this work were carried out for Calabi-Yau threefolds with an understanding 
that an orientifold involution still needs to be implemented to obtain a minimally supersymmetric effective theory. A more elegant way to directly obtain an $\cN=1$ effective theory is to consider F-theory compactifications on elliptically fibered Calabi-Yau fourfolds. Remarkably, the used asymptotic Hodge theory methods are equally applicable to these higher-dimensional manifolds. In fact, we expect that these methods open the way to study interesting moduli stabilization schemes for F-theory as recently demonstrated in \cite{Grimm:2019ixq,Grimm:2020ouv} and \cite{Marchesano:2021gyv}. We believe that this novel way of studying F-theory flux vacua sets us on the track to understand the structure of the flux landscape, sidetracking the fact that only a sparse number of explicit period computations for Calabi-Yau fourfolds has been performed.  




\begin{subappendices}

\section{Flux vacua near finite distance points} \label{finite_distance_appendix}

In this appendix we study flux vacua with exponentially small superpotentials near finite distance boundaries in complex structure moduli space, i.e.~type $\mathrm{I}$ points. We explain that the strategy laid out in section \ref{ssec:strategy} does not stabilize all moduli for such boundaries, and exponential corrections to the polynomial scalar potential $V_{\rm pol}$ are needed to lift flat directions.

Let us begin by inspecting the constraints put by the vanishing of the polynomial superpotential and the F-term of the axio-dilaton $\tau$ at the vacuum. These conditions together can be conveniently rewritten as
\begin{equation}
\langle F_3, \, \Pi_{\rm pol} \big|_* \rangle = 0 \, , \qquad \langle H_3,\,  \Pi_{\rm pol} \big|_* \rangle = 0 \, .
\end{equation}
Recall now that we can expand these polynomial periods as $ \Pi_{\rm pol} = e^{t^iN_i}a_0$, and subsequently use that $N_i a_0=0$ for type $\mathrm{I}$ points, giving $ \Pi_{\rm pol} = a_0$. It then follows that the polynomial part of the superpotential vanishes identically, i.e.~for any values of the axio-dilaton and the complex structure moduli we must have
\begin{equation}
W_{\rm pol} = \langle F_3 -\tau H_3, \, a_0 \rangle =  0\, ,
\end{equation}
since both $\langle F_3 , a_0 \rangle=0$ and $ \langle  H_3, a_0 \rangle  = 0$. Note that requiring $D_\tau W_{\rm pol}=0$ for these vacua thus only imposes a constraint on the fluxes $F_3$ and $H_3$, and in particular does not fix any of the moduli. Furthermore, corrections to this F-term through $D_\tau W_{\rm inst}$ only enter the scalar potential \eqref{eq:potential} at exponential order, since $K^{\tau \bar{\tau}}$ is polynomial in the fields. In contrast, metric-essential instantons cause the inverse K\"ahler metric $K^{i \bar{j}}$ to have $h^{2,1}$ exponentially large eigenvalues for finite distance boundaries, so the complex structure moduli F-terms $D_i W_{\rm inst}$ do contribute to the polynomial scalar potential. The polynomial scalar potential therefore reduces to
\begin{equation}
V_{\rm pol} = \frac{1}{\cV^2} e^K K^{i \bar{j}} D_i W_{\rm inst} D_{\bar{j}} \bar{W}_{\rm inst}\, ,
\end{equation}
where the indices $i,j$ run only over complex structure moduli. The crucial observation is now that the polynomial scalar potential is minimized by imposing $D_i W_{\rm inst}=0$. This yields only $h^{2,1}$ constraints on the complex structure moduli and axio-dilaton, leaving us with one free modulus. In principle one can lift this flat direction by including exponential corrections to the polynomial scalar potential $V_{\rm pol}$. In fact, to some extent we have control over these corrections, since non-metric essential instantons and $D_\tau W_{\rm inst}$ enter the scalar potential at exponential order. However, one might find that for instance non-essential instantons compete with these corrections to the scalar potential. Furthermore, even if the effective potential for this polynomially flat direction can be determined, the resulting extremization conditions will be of a much more complicated form than the algebraic equations \eqref{eq:polextr} and \eqref{eq:expextr} we encountered previously. For this reason we leave the search for flux vacua with exponentially small superpotentials near finite distance boundaries to future work. 

\end{subappendices}
